Realizing holonomic constraints in classical and quantum mechanics

We consider the problem of constraining a particle to a submanifold Sigma of configuration space using a sequence of increasing potentials. We compare the classical and quantum versions of this procedure. This leads to new results in both cases: an unbounded energy theorem in the classical case, and a quantum averaging theorem. Our two step approach, consisting of an expansion in a dilation parameter, followed by averaging in normal directions, emphasizes the role of the normal bundle of Sigma, and shows when the limiting phase space will be larger (or different) than expected.

==> Constraints.tex <==
\input rixmax
\def\ss{{\bf \sigma}}
\def\SS{{\Sigma}}
\def\nn{{\bf n}}
\def\xx{{\bf x}}
\def\yy{{\bf y}}
\def\vv{{\bf v}}
\def\e{{\bf e}}
\def\tr{{\rm tr}}
\def\aj{{\alpha,j}}
\def\bk{{\beta,k}}
\def\Lsl{L_{\sharp \lambda}}
\def\Ll{L_\lambda}

\def\HBbar{\overline{H}_B}

\def\Rsl{R_{\sharp \lambda}}
\def\Rl{R_\lambda}
\def\tocome{\vskip 20pt \hrule\vskip 20pt\centerline{$\ldots$still to come$\ldots$} \vskip 20pt \hrule\vskip 20pt}
\def\shd#1{\hd{\the\secnumber. #1}}
%\input epsf
%\draftmode
\def\mcomment#1{}
%\magnification 1100
	\hsize = 5.9 true in
	\hoffset = 0.45 true in
	\baselineskip = 18pt
\font\tenrm=pplr at 9.5pt
\font\tensl=pplro at 9.5pt
\font\eightit=pplri at 8.5 pt
%\font\tenrm=cmr10 at 9.5pt
%\font\tensl=cmsl10 at 9.5pt
%\font\bold=cmssbx10 at 10pt
\tenrm	

%\def\mcomment#1{}
\footline={\hfil}
\footline={\hss\tenrm\folio\hss}
\def\half{{{1}\over{2}}}
\def\SS{{\Sigma}}

\centerline{\bold Realizing holonomic constraints}
\vskip 10 pt 
\centerline{\bold in classical and quantum mechanics}
\vskip 20 pt

\centerline{Richard Froese}
\medskip
\centerline{Department of Mathematics}
\centerline{University of British Columbia}
\centerline{Vancouver, British Columbia, Canada}
\vskip 20pt
\centerline{and}
\vskip 20 pt
\centerline{Ira Herbst}
\medskip
\centerline{Department of Mathematics}
\centerline{University of Virginia}
\centerline{Charlottesville, Virginia, USA}
\vskip 20pt
\centerline{\today}
\vskip 20pt


\vskip 20 pt
\input abstract
\input intro
\input results
\input quantum
\input coords
\input classical1
\input classical2
\input coords2
\input quantumpf1
\input quantumpf2
\input refs

\rixend


==> abstract.tex <==
\font\ninesl=pplro at 9.0pt

\centerline{\bold Abstract}

\quote{\ninesl
We consider the problem of constraining a particle to a submanifold $\Sigma$
of configuration space using a sequence of increasing potentials. We compare the classical and quantum versions of this procedure. This leads to new results in both cases: an unbounded energy theorem in the classical case, and a quantum averaging theorem. Our two step approach, consisting of an expansion in a dilation parameter, followed by averaging in normal directions, emphasizes the role of the normal bundle of $\Sigma$, and shows when the limiting phase space will be larger (or different) than expected.
}


==> classical1.tex <==
%\vfill\eject
\beginsection
\shd{Proofs of theorems in classical mechanics}

\beginproofof{\thmrf{classical1}} We begin with some remarks about the co-ordinate charts for $T^*N\SS$. 
We will assume that the frames used to defined the co-ordinates consist of eigenvectors of $A(\ss)$.
We assume that each chart has the form $\{(\ss,n,\xi,\eta): \ss\in\UU, n\in N_\ss\SS, \xi\in T^*_{\ss,n}N\SS \hbox{ is horizontal}, \eta \in T^*_{\ss,n}N\SS \hbox{ is vertical}\}$, where $\UU$ is a co-ordinate
chart for $\SS$. 
Since $\SS$ is compact, there is an atlas with finitely many charts, and there exists a positive number
$\epsilon_1$ so that two points in $T^*N\SS$ both lie in a single chart if their projections onto $\SS$ are a distance
less than $\epsilon_1$ apart.

We use the notation
$$
\gamma_\lambda(t) = \phi^{L_\lambda}_t(\gamma_\lambda), \quad \gamma^\lambda(t) = \phi^{H_B+\lambda^2 H_0}_t(\gamma_0).
$$

Our first estimates are large ${\lambda}$ bounds on the components of  
$$
\gamma_\lambda(t)=(\ss_\lambda(t),n_\lambda(t),\xi_\lambda(t),\eta_\lambda(t))
$$ 
that follow from the conservation of energy.
These bounds are
\be{energybdds1}
|n_\lambda(t)|, |\eta_\lambda(t)| \le C
\ee
and
\be{energybdds2}
|\xi_\lambda(t)| \le C{\lambda}
\ee
The analogous bounds also hold for $\gamma^\lambda(t)=(\ss^\lambda(t),n^{\lambda}(t),\xi^{\lambda}(t),\eta^{\lambda}(t))$. 
Clearly $|n_\lambda(t)| = |y_\lambda(t)|$ and, by \rf{etanorm}, $|\eta_\lambda(t)|=|r_\lambda(t)|$. Thus,
\rf{energybdds1} implies that
$|y_\lambda(t)|$ and $|r_\lambda(t)|$ remain bounded. 

To prove these we first consider the action of $D_{\lambda}^{-1}$ on
$\xi_\lambda$. Let $\gamma_\lambda=(\ss_\lambda,n_\lambda,\xi_\lambda,\eta_\lambda)$ have co-ordinates
$(x_\lambda,y_\lambda,p_\lambda,r_\lambda)$. Then $\xi_\lambda\in T^*_{\ss_\lambda,n_\lambda}N\SS$ has co-ordinates
$$
P^H\left[\matrix{p_\lambda\cr r_\lambda\cr}\right] = \left[\matrix{p_\lambda-B(x_\lambda,y_\lambda)r_\lambda\cr 0\cr}\right]
$$
We now wish to apply $D_{\lambda}^{-1}$.
Since $B(x,y)$ is linear in $y$, the scaling in $y_\lambda$ and in $r_\lambda$ cancel. In other words
$$
B(x_\lambda,{\lambda}^{-1}y_\lambda){\lambda} r_\lambda=B(x_\lambda,y_\lambda)r_\lambda.
$$
Thus $D_{\lambda}^{-1}\xi_\lambda\in T^*_{\ss_\lambda,{\lambda}^{-1}n_\lambda}N\SS$ has the same co-ordinates as  $\xi_\lambda\in T^*_{\ss_\lambda,n_\lambda}N\SS$. 
This implies that as $\lambda\rarr\infty$,
\be{Dlxi}\eqalign{
|D_{\lambda}^{-1}\xi_\lambda|^2 &= \left\langle\left[\matrix{p_\lambda-B(x_\lambda,y_\lambda)r_\lambda\cr 0\cr}\right],G^{-1}(x_\lambda,{\lambda}^{-1}y_\lambda)\left[\matrix{p_\lambda-B(x_\lambda,y_\lambda)r_\lambda\cr 0\cr}\right]\right\rangle\cr
&=\jap{\big(p_\lambda-B(x_\lambda,y_\lambda)r_\lambda\big),\big(G_\SS(x_\lambda)+C(x_\lambda,{\lambda}^{-1}y_\lambda)\big)^{-1}\big(p_\lambda-B(x_\lambda,y_\lambda)r_\lambda\big)}\cr
&\rarr \jap{\big(p_0-B(x_0,y_0)r_0\big),G_\SS(x_0)^{-1}\big(p_0-B(x_0,y_0)r_0\big)}\cr
&=|d\pi^{*-1}\xi_0|^2
}\ee
Thus, for large $\lambda$, the initial energy satisfies
$$\eqalign{
L_{\lambda}(\gamma_\lambda)=H_{\lambda}\circ D_{\lambda}^{-1}(\gamma_\lambda) 
&\le \half |D_{\lambda}^{-1}\xi_\lambda|^2 + C_V
+ {{{\lambda^2}}\over{2}}\left(|\eta_\lambda|^2 + \jap{n_\lambda,A(\ss_\lambda) n_\lambda)}\right)\cr
&\le C{\lambda^2},
}$$
where $C_V$ is an upper bound for $V$ in a neighbourhood of $\SS$. Given this bound on the initial
energies, we may assume that $V$ is bounded, as was explained in the introduction.
We now estimate  the energy for later times $t$.
$$\eqalign{
L_{\lambda}(\gamma_\lambda(t))=H_{\lambda}\circ D_{\lambda}^{-1}(\gamma_\lambda(t)) 
&\ge \half|D_{\lambda}^{-1}\xi_\lambda(t)|^2 - \|V\|_\infty
+ C{\lambda^2}\left(|\eta_\lambda(t)|^2 + |n_\lambda(t)|^2\right)\cr
&\ge - \|V\|_\infty
+ C{\lambda^2}\left(|\eta_\lambda(t)|^2 + |n_\lambda(t)|^2\right)\cr
}$$
Since energy is conserved, i.e., $L_{\lambda}(\gamma_\lambda(t))=L_{\lambda}(\gamma_\lambda)$, this implies \rf{energybdds1}. In a similar way we find that
\be{Dlbdd}
|D_{\lambda}^{-1}\xi_\lambda(t)|^2\le C{\lambda^2}.
\ee
Now for $|y| < C_1$ sufficiently large $\lambda$ there is a constant $C$ such that
$$
G^{-1}(x,y) < CG^{-1}(x,{\lambda}^{-1}y)
$$
in any of the finitely many co-ordinate patches.
Thus, \rf{Dlxi} implies
$$
|\xi_\lambda(t)| \le |D_{\lambda}^{-1}\xi_\lambda(t)|,
$$
so that \rf{Dlbdd} implies \rf{energybdds2}.

The proof of bounds
\rf{energybdds1} and \rf{energybdds2} for $\gamma^\lambda(t)$ is similar.

We now wish to improve the bound \rf{energybdds2} to
\be{impbdds2}
|\xi_\lambda(t)| \le C
\ee
for $0\le t\le T$. 
We begin by defining a function $Q$ that depends on our co-ordinate systems.
Let $\chi_1(\ss),\ldots, \chi_N(\ss)$ be a partition of unity with each
$\chi_k$ supported in a single co-ordinate patch. Define $Q=\sum Q_k\chi_k$,
where the local co-ordinate expression for $Q_k$ is 
$$
Q_k(x,p) = \half\jap{p,G_\SS(x)^{-1}p} + 1.
$$
(We are abusing notation by using the same letter $Q_k$ for the function on $T^*N\SS$ and its
local co-ordinate expression.) Given \rf{energybdds1} we may find a constant $C$ such that
$$
|\xi_\lambda(t)|^2 \le C Q(\gamma_\lambda(t))
$$
Thus bound \rf{impbdds2} follows from an upper bound for $Q$ along an orbit. 

To establish such a bound we first estimate the time derivative of  $Q_k(x_\lambda(t),p_\lambda(t))$.
This derivative
is given by the Poisson bracket.
$$
{{d}\over{dt}} Q_k(x_\lambda(t),p_\lambda(t)) = \left\{Q_k,L_{\lambda}\right\}(x_\lambda(t),p_\lambda(t),p_\lambda(t),r_\lambda(t))
$$
Recall that the orthonormal frame $n_1(\ss),\ldots,n_m(\ss)$ giving our local co-ordinates  consists of eigenvectors 
of $A(\ss)$. Thus
$$
L_{\lambda} = H_B + {\lambda^2} H_O + E_{\lambda}
$$
with
$$
H_B(x,y,p,r) = Q_k(x,p) - \jap{B(x,y)r, G_\SS(x)^{-1}p} + {{1}\over{2}}\jap{B(x,y)r, G_\SS(x)^{-1}B(x,y)r} + V(x,0), 
$$
$$
H_O(x,y,p,r) = \half\jap{r,r} + \half\sum_i\omega_i^2 y_i^2
$$
and
$$\displaylines{\quad
E_{\lambda}(x,y,p,r) =  \hfill\cr\hfill
\eqalign{
& {{1}\over{2}}\left\langle
\Big(p-B(x,y)r\Big),
\Big((G_\SS(x)+C(x,{\lambda}^{-1}y))^{-1}-G_\SS(x)^{-1}\Big)
\Big(p-B(x,y) r\Big)
\right\rangle
\cr
&\quad +V(x,{\lambda}^{-1}y)-V(x,0)\cr}
\quad\cr}$$
Since $Q_k$ only depends on $x$ and $p$ any Poisson bracket $\{Q_k, F\}$ is given in local co-ordinates
by
$$
\{Q_k, F\} = \sum_i {{\PA Q_k}\over{\PA p_i}}{{\PA F}\over{\PA x_i}}-
{{\PA Q_k}\over{\PA x_i}}{{\PA F}\over{\PA p_i}}.
$$
Thus $\{Q_k,H_O\}=\{Q_k,Q_k\}=0$. Using these formulas, together with \rf{energybdds1}
and \rf{energybdds2} we find
\be{Qdot}\eqalign{
{{d}\over{dt}} Q_k(x_\lambda(t),p_\lambda(t)) &\le 
C\left(\|p_\lambda(t)\|^2 + {\lambda}^{-1}\|p_\lambda(t)\|^3\right)\cr
&\le C Q_k(x_\lambda(t),p_\lambda(t))
}\ee

Next, writing Hamilton's equations for $x_\lambda(t)$ and using \rf{energybdds1} we find
\be{xdotbdd}\eqalign{
|\dot x_\lambda(t)| &\le \left|{{\PA H_B}\over{\PA p}}\right|\cr
&\le C Q^{\half}(x_\lambda(t),p_\lambda(t))\cr
}\ee
Since the cutoff functions, written in local co-ordinates, only depend on  $x_\lambda$ we find
that
\be{chibdd}
|\dot\chi_k| \le C |\dot x_\lambda| \le C Q^\half
\ee


Now we show if we evaluate $Q_k$ and $Q_j$ at the same point $\gamma=(\ss,n,\xi,\eta)$ with
$|n|,|\eta| < C$ then
\be{Qijbdd}
|Q_k(\gamma)- Q_j(\gamma)| \le C Q_k(\gamma)^\half.
\ee 
To see this, we first compute how our co-ordinates change. If $(\tilde x, \tilde y,\tilde p,\tilde r)$
are the  co-ordinates in the $j$th chart, obtained from the co-ordinates in the $i$th chart
by a 
change of co-ordinates on $\SS$ and a change of frame, then
$$\eqalign{
\tilde p &= Mp + b\cr
\tilde G_\SS^{-1} &= M^{-1}G_\SS^{-1}M^{-1}
}$$
where $M$ is the $n\times n$ matrix with entries $\PA \tilde x_i / \PA x_j$ and $b$ is a vector with components
$\sum r_k y_l \PA \theta_{kl}/\PA x_i $ for an orthogonal matrix valued function $\theta(x)$ given by
taking inner products of the elements of the old and new frames. Thus
$$\eqalign{
Q_j &= \jap{\tilde p, \tilde G_\SS^{-1}\tilde p} + 1\cr
&= Q_k + 2\jap{b,M^{-1}G_\SS^{-1}p} + \|b\|^2 + 1\cr
&\le Q_k + C Q_k^\half \cr
}$$
This implies \rf{Qijbdd}.

Now we are ready to establish a bound for $Q$ along an orbit. Let $\dot Q$ denote $dQ(\gamma_\lambda(t))/dt$. 
Then
$$
\eqalign{
\dot Q &= \sum_j \dot Q_j\chi_j + Q_j\dot\chi_j \cr
&= \sum_j \dot Q_j\chi_j + \sum_{k,j}Q_j\dot\chi_j\chi_k \cr
}$$
The first term is estimated using \rf{Qdot} yielding
$$
\sum_j \dot Q_j\chi_j \le C \sum_j  Q_j\chi_j =CQ
$$
To estimate the second term, note that since $\sum_k \chi_k = 1$,
we have $\sum_k \dot\chi_k = 0$. Thus 
$$
\sum_{k,j}Q_k\dot\chi_j\chi_k = 0
$$
so that
$$\eqalign{
\sum_{k,j}Q_j\dot\chi_j\chi_k &= \sum_{k,j}(Q_j-Q_k)\dot\chi_j\chi_k\cr
&\le CQ
}$$
by \rf{chibdd} and \rf{Qijbdd}. Thus we have the differential inequality
$$
\dot Q \le C Q
$$
which implies
$$
Q(\gamma_\lambda(t)) \le Q(\gamma_\lambda(0))e^{Ct}
$$
This implies \rf{impbdds2}




Note that \rf{xdotbdd} implies
\be{sigmabdd}
\|\dot\ss_\lambda(t)\|, \|\dot\ss^\lambda(t)\| < C
\ee
for $0\le t \le T$. 

We will now show that there exists $\epsilon >0$ such that if
\be{lamlim}
\lim_{\lambda\rarr\infty}\sup_{\tau\in[0,t]}\|\gamma_\lambda(\tau)-\gamma^\lambda(\tau)\|=0
\ee
holds for some $t=t_1 \le T$ then \rf{lamlim} also holds for any $t\le t_1+\epsilon$.
Since \rf{lamlim} holds for $t=0$ by the assumption on the initial conditions, this will complete
the proof.

So assume that \rf{lamlim} holds for $t=t_1 \le T$. To compare the two orbits for
nearby times, we want to ensure that they lie in the same co-ordinate patch. 
There exists an $\epsilon_1>0$ such that $\gamma_\lambda$ and $\gamma^\lambda$ will lie in the same co-ordinate chart if $\|\ss_\lambda-\ss^\lambda\|<\epsilon_1$.

Choose $\lambda_0$ so that $\lambda > \lambda_0$ implies
$$
\sup_{\tau\in[0,t_1]}\|\gamma_\lambda(\tau)-\gamma^\lambda(\tau)\| < \epsilon_1/3
$$
Now fix $j>j_0$. For $t>t_1$
$$\eqalign{
\|\ss_\lambda(t)-\ss^\lambda(t)\| &\le \|\ss_\lambda(t)-\ss_\lambda(t_1)\|+\|\ss_\lambda(t_1)-\ss^\lambda(t_1)\|
+\|\ss^\lambda(t_1)-\ss^\lambda(t)\|\cr
&\le 2|t-t_1|C + \epsilon_1/3\cr
}$$
where $C$ is the constant from \rf{sigmabdd}. Thus if we choose $\epsilon < \epsilon_1/3C$ then $\gamma_\lambda$ and $\gamma^\lambda$ 
will lie in the same co-ordinate chart for $t\in [t_1,t_1+\epsilon]$. Notice that we do not rule out the the chart changes with $\lambda$.

We now write down the differential equation for $\gamma_\lambda$ and $\gamma^\lambda$ in this common co-ordinate chart. 
Let $z\in\RR^{2(n+m)}$ denote co-ordinates for $T^*N\SS$, i.e.,
$$
z = \left[\matrix{ x\cr y\cr p\cr r\cr}\right].
$$
Denote by $z_\lambda$ the co-ordinates of $\gamma_\lambda$ and by $z^\lambda$ the co-ordinates of $\gamma^\lambda$.
For a Hamiltonian $H$, let $X_H$ denote the corresponding Hamiltonian vector field given in local co-ordinates
by
%$$
%X_H(z) = \left[\matrix{\displaystyle{{\PA H}\over{\PA x}}(z)\cr \displaystyle{{\PA H}\over{\PA y}}(z)\cr -\displaystyle{{\PA %H}\over{\PA p}}(z)\cr -\displaystyle{{\PA H}\over{\PA r}}(z)\cr }\right]
%$$
$$
X_H(z) = \left[\matrix{\phantom{-}\PA H/\PA x(z)\cr \phantom{-}\PA H/\PA y(z)\cr -\PA H/\PA p(z)\cr -\PA H/\PA r(z)\cr}\right]
$$
Then
\be{evolution}
{{d}\over{dt}}z_\lambda(t)
= X_{H_B}\left(z_\lambda(t)\right) 
+ X_{{\lambda^2}H_O}\left(z_\lambda(t)\right)
+ X_{E_{\lambda}}\left(z_\lambda(t)\right)
\ee
Since $H_O$ is quadratic, the vector field $X_{{\lambda^2}H_O}$ is linear, given by
$$
X_{{\lambda^2}H_O}\left(z\right)
= {\lambda^2} Dz
$$
for a matrix $D$ that is similar to a real antisymmetric matrix. It follows that \rf{evolution} can be written in integral form
$$
z_\lambda(t)
=e^{{\lambda^2} (t-t_1) D}z_\lambda(t_1)
+ e^{{\lambda^2} t D}\int_{t_1}^t e^{-{\lambda^2} \tau D}\Big(
X_{H_B}\left(z_\lambda(\tau)\right)
+X_{E_{\lambda}}\left(z_\lambda(\tau)\right)\Big) d\tau
$$
We may write a similar equation for the co-ordinates of $\gamma^\lambda$ and obtain
$$\displaylines{\quad
z_\lambda(t)-z^\lambda(t)
=
e^{{\lambda^2} (t-t_1) D}(z_\lambda(t_1)-z^\lambda(t_1))
\hfill\cr\hfill
+ e^{{\lambda^2} t D}\int_{t_1}^t e^{-{\lambda^2} \tau D}\Big(
X_{H_B}\left(z_\lambda(\tau)\right)
-X_{H_B}\left(z^\lambda(\tau)\right)
+X_{E_{\lambda}}\left(z_\lambda(\tau)\right)\Big) d\tau
\quad}$$
The harmonic oscillator evolution $e^{{\lambda^2} t D}$ is similar to a rotation and therefore uniformly bounded.
Moreover we have the estimates
$$
\left\|
X_{H_B}\left(z_\lambda(\tau)\right)
-X_{H_B}\left(z^\lambda(\tau)\right)
\right\|
\le C
\left\|
z_\lambda(\tau)-z^\lambda(\tau)
\right\|
$$
and
$$
\left\|
X_{E_{\lambda}}\left(z_\lambda(\tau)\right)
\right\|
\le C{\lambda}^{-1}
$$
These follow from \rf{energybdds1} and \rf{impbdds2} which imply that the co-ordinates for the orbits stay in 
compact sets. Thus
$$
\left\|
z_\lambda(t)-z^\lambda(t)
\right\|
=
C\left\|
z_\lambda(t_1)
-z^\lambda(t_1)
\right\|
+ C |t-t_1|\sup_{\tau\in[t_1,t_1+\epsilon]}\left\|
z_\lambda(\tau)
-z^\lambda(\tau)
\right\| +C |t-t_1|{\lambda}^{-1}
$$
If we now also insist that 
$$
\epsilon < 1/(2C)
$$
then we find that
$$
\half \sup_{\tau\in[t_1,t_1+\epsilon]}\left\|z_\lambda(\tau)-z^\lambda(\tau)\right\|
\le C\left\|z_\lambda(t_1)-z^\lambda(t_1)\right\| + C \epsilon{\lambda}^{-1}
$$
Since we have only finitely many co-ordinate charts, there is a constant $C$ so that
$$
C^{-1} \left\|z_\lambda(\tau)-z^\lambda(\tau)\right\| 
\le \|\gamma_\lambda(\tau) - \gamma^\lambda(\tau)\| 
\le C \left\|z_\lambda(\tau)-z^\lambda(\tau)\right\|
$$ in any chart.
Thus we conclude that
$$
\sup_{\tau\in[t_1,t_1+\epsilon]} \|\gamma_\lambda(\tau) - \gamma^\lambda(\tau)\| \le C\left\|\gamma_\lambda(t_1)-\gamma^\lambda(t_1)\right\|+C \epsilon{\lambda}^{-1}
$$
This implies that 
$$
\lim_{\lambda\rarr\infty}\sup_{\tau\in[t_1,t_1+\epsilon]} \|\gamma_\lambda(\tau) - \gamma^\lambda(\tau)\|=0
$$
and completes the proof.

\endproof





==> classical2.tex <==
\beginproofof{\thmrf{classical2}}
We will show that there exists $\epsilon > 0$ such that if \rf{cl2est} holds for some $t=t_1\le T$,
then \rf{cl2est} also holds for any $t\le t_1+\epsilon$. So assume that \rf{cl2est} holds for some $t=t_1\le T$.

Define
$$
\psi_\lambda(t) = \phi_{-t}^{\lambda^2H_O}\circ\phi_t^{H_B+\lambda^2H_O}(\gamma_0)
$$
Choosing our co-ordinate charts as in the proof of \thmrf{classical1}, we find that for 
small enough $\epsilon$, $\psi_\lambda(t)$ will stay in a single chart for $t\in[t_1,t_1+\epsilon]$.
This follows from the estimate \rf{sigmabdd} for $\gamma^\lambda(t)=\phi_t^{H_B+\lambda^2H_O}(\gamma_0)$
and the fact that the harmonic oscillator motion $\phi_{-t}^{\lambda^2H_O}$ keeps the base point $\sigma$ fixed.

Let $w_\lambda(t)$ denote the local co-ordinates of $\psi_\lambda(t)$. In local co-ordinates,
the evolution $\phi_{-t}^{\lambda^2H_O}$ is given by multiplication by $e^{-t\lambda^2 D}$, and
so
$$
w_\lambda(t) = e^{-t\lambda^2 D}z^\lambda(t),
$$
where $D$ is the same matrix, similar to a real antisymmetric matrix, that appeared in the proof of \thmrf{classical1}, 
and $z^\lambda(t)$ are the co-ordinates of $\gamma^\lambda(t)$. Differentiating, we obtain
$$\eqalign{
{{dw_\lambda(t)}\over{dt}} &= e^{-t\lambda^2 D}X_{H_B}(e^{t\lambda^2 D}w_\lambda(t)),\cr
%&= X_{H_B\circ\phi_{t}^{\lambda^2H_O}}(w_\lambda(t))\cr
}$$
so that for $t\in [t_1,t_1+\epsilon]$,
\be{intw}
w_\lambda(t) = w_\lambda(t_1) + \int_{t_1}^t e^{-s\lambda^2 D}X_{H_B}(e^{s\lambda^2 D}w_\lambda(s)) ds
\ee

Now consider the family of $\RR^{2(n+m)}$ valued functions on $[t_1,t_1+\epsilon]$ given by ${\cal W}=\{w_\lambda(\cdot) : \lambda > 0\}$.
We will show for any sequence $\lambda_j\rarr\infty$, there is a subsequence $\lambda_{1,j}$ such that $w_{\lambda_{1,j}}$ converges
uniformly to the same limit $w_\infty$. This will imply that $w_\lambda \rarr w_\infty$ uniformly.

The estimates \rf{energybdds1} and \rf{impbdds2} of \thmrf{classical1} and the fact that the matrices $e^{-t D}$
are bounded uniformly  in $t$ imply that ${\cal W}$ is a bounded family. Moreover, from \rf{intw} and the boundedness
of the orbits, it follows that
$$
\|w_\lambda(t)-w_\lambda(t')\| \le C|t-t'|
$$
so that ${\cal W}$ is equicontinuous. Suppose we are given a sequence $\lambda_j\rarr\infty$. Then, by Ascoli's theorem, there exists
subsequence $\lambda_{1,j}$ so that $w_{\lambda_{1,j}}$ converges uniformly to $w_{\infty}$. We wish to show that $w_{\infty}$ is always
the same, no matter which sequence we start with.  Our assumption on $t_1$ implies that $w_{\lambda_{1,j}}(t_1)$ always converges to the same $w_0$, namely to the co-ordinates of $\phi_{t_1}^{\HBbar}(\gamma_0)$. We will show that $w_\infty(t)$ is the orbit generated by the Hamiltonian $\HBbar$ with initial condition $w_0$ at $t=t_1$. 


Using the uniform boundedness of the matrices $e^{-t D}$ in \rf{intw} we find that
$$
w_\infty(t) = w_0 + \int_{t_1}^t e^{-s\lambda_{1,j}^2 D}X_{H_B}(e^{s\lambda_{1,j}^2 D}w_\infty(s)) ds + o(1)
$$
as $j\rarr\infty$. Now $e^{s\lambda_{1,j}^2 D}$ is a symplectic map, being the Hamiltonian flow $\phi_{s\lambda_{1,j}^2}^{H_0}$ in local co-ordinates. It 
follows that
$$
e^{-s\lambda_{1,j}^2 D}X_{H_B}(e^{s\lambda_{1,j}^2 D}w_\infty(s)) = X_{H_B\circ\phi_{s\lambda_{1,j}^2}^{H_0}}(w_\infty(s))
$$
If we use the Fourier expansion
$$
H_B\circ\phi_{s\lambda_{1,j}^2}^{H_0} = \sum_{\nu\in\ZZ^{m_0}} e^{is\lambda_{1,j}^2\jap{\nu,\omega}} F_\nu
$$
we find that
$$
X_{H_B\circ\phi_{s\lambda_{1,j}^2}^{H_0}} = \sum_{\nu\in\ZZ^{m_0}}e^{is\lambda_{1,j}^2\jap{\nu,\omega}} X_{F_\nu}
$$
so that
$$
w_\infty(t) = w_0 + \sum_{\nu\in\ZZ^{m_0}}\int_{t_1}^t e^{is\lambda_{1,j}^2\jap{\nu,\omega}} X_{F_\nu}(w_\infty(s)) ds + o(1)
$$
Taking $j$ to infinity and using the Riemann-Lebesgue lemma, we find that
$$\eqalign{
w_\infty(t) &= w_0 + \sum_{\nu\in\ZZ^{m_0}:\jap{\nu,\omega}=0}\int_{t_1}^t X_{F_\nu}(w_\infty(s)) ds\cr
&=w_0 + \int_{t_1}^t X_{\HBbar}(w_\infty(s)) ds\cr
}$$
This identifies $w_\infty(t)$ as the orbit generated by $\HBbar$ with initial condition $w_0$ at $t_1$, as claimed.


Now we have
$$
\sup_{t\in[t_1,t_1+\epsilon]}\left\|e^{-t\lambda^2D}z^\lambda(t) - w_\infty(t)\right\| \rarr 0
$$
as $\lambda\rarr\infty$ which implies
$$
\sup_{t\in[t_1,t_1+\epsilon]}\left\|z^\lambda(t) - e^{t\lambda^2D}w_\infty(t)\right\|  \rarr 0
$$
This implies
$$
\sup_{t\in[t_1,t_1+\epsilon]}\left\|\phi^{H_B+\lambda^2 H_0}_t(\gamma_0) 
			- \phi^{\lambda^2 H_0}_t\circ\phi^{\HBbar}_t(\gamma_0)\right\|\rarr 0
$$
and completes the proof.
\endproof
\endsection


==> coords.tex <==
\beginsection
\def\nn{n}
\shd{Co-ordinate expressions}

Our proofs will rely on local co-ordinate expressions for the quantities introduced above. 

Suppose $x(\ss)$ is a local co-ordinate map for $\SS$. Its inverse $\ss(x)$ is 
a local imbedding of $\RR^n$ onto $\SS\subset\RR^{n+m}$. Given a local orthonormal frame $n_1(\ss),\ldots,n_m(\ss)$ for 
the normal bundle, we obtain
local co-ordinates for $N\SS$ by setting 
$$\eqalign{
x_i(\ss,n) &= x_i(\ss), \quad i=1,\ldots,n \cr
y_i(\ss,n) &= \jap{n_i(\ss),n}, \quad i=1,\ldots,m \cr
}$$
We then may form the standard bases $\PA/\PA x_1,\ldots,\PA/\PA x_n,\PA/\PA y_1,\ldots,\PA/\PA y_m$ for 
the tangent spaces of $N\SS$ and $dx_1,\ldots,dx_n,dy_1,\ldots,dy_n$ for the cotangent spaces. This gives rise
to local co-ordinates for $TN\SS$ and $T^*N\SS$ in the standard way. For the cotangent bundle, we will
denote these by $(x,y,p,r)\in\RR^{2(n+m)}$. Thus $(x,y,p,r)$ denotes the cotangent vector $\sum p_i dx_i + \sum r_j dy_j$ in
the cotangent space over $(\ss(x),\sum_j y_j n_j(\ss))$.

The standard symplectic form for $T^*N\SS$ is the two form given by 
$$
\omega = \sum_{i=1}^n dp_i\wedge dx_i + \sum_{j=1}^m dr_j\wedge dy_j
$$

The dilation map $D_\lambda$ is given in local co-ordinates by
\be{Dlc}
D_\lambda(x,y,p,r) = (x,\lambda y,p,\lambda^{-1}r)
\ee
Clearly this map preserves the symplectic form $\omega$.


We now compute the local expression for the metric. Let $\ss_i(x)\in\RR^{n+m}$ denote the vector $\PA\ss(x)/\PA x_i$.
The tangent vector $\PA/\PA x_i\in T_{(\ss,n)}N\SS$ corresponds to
the vector in $\RR^{2(n+m)}$ given by $(\ss_i, \sum_j y_j dn_j(\ss)[\ss_i])$. The tangent vector $\PA/\PA y_j$ corresponds to $(0,n_j(\ss))$
Here $\ss=\ss(x)$, $\ss_i=\ss_i(x)$ and $n=\sum_j y_jn_j(\ss(x))$. Using  \rf{ip} for the inner product, we find
that the local expression for the metric has block form
\be{Gblock}
G(x,y) = \left[\matrix{G_\SS+C+BB^T&B\cr B^T&I\cr}\right] 
= \left[\matrix{I&B\cr 0&I\cr}\right]\left[\matrix{G_\SS+C&0\cr 0&I\cr}\right]\left[\matrix{I&B\cr 0&I\cr}\right]^T
\ee
where $G_\SS=G_\SS(x)$ is the metric for $\SS$ with matrix entries $\jap{\ss_i(x),\ss_j(x)}$,
$B=B(x,y)$ is the matrix with entries
\be{Bmat}
B_{i,j}(x,y) = \sum_k y_k\jap{d\nn_k[\ss_i],\nn_j}
\ee
and
where $C=C(x,y)$ is the matrix with entries
\be{Cmat}\eqalign{
C_{i,j}(x,y) &= \sum_k y_k (\jap{d\nn_k[\ss_i],\ss_j}+\jap{\ss_i,d\nn_k[\ss_j]}) + \sum_{k,l} y_ky_l\jap{dn_k[\ss_i],dn_l[\ss_j]} - BB^T\cr
&=\sum_k y_k (\jap{d\nn_k[\ss_i],\ss_j}+\jap{\ss_i,d\nn_k[\ss_j]}) + \sum_{k,l} y_ky_l\jap{dn_k[\ss_i],P^T_\ss dn_l[\ss_j]}\cr
}\ee
The geometrical meaning of the term $G_\SS + C$ is given in \rf{GplusC} below.

The inverse can be written
\be{Ginvblock}
G^{-1}(x,y) = \left[\matrix{I&-B\cr 0&I\cr}\right]^T\left[\matrix{(G_\SS+C)^{-1}&0\cr 0& I}\right]\left[\matrix{I&-B\cr 0&I\cr}\right]
\ee

The local expressions for the projections onto the vertical and horizontal subspaces can now be computed. 
Let $P_V$ and $P_H$ denote the projections for the tangent space and $P^V$ and $P^H$ the projections for the 
cotangent spaces. Then
$$
P_V=\left[\matrix{0& 0\cr B^T & I\cr}\right]\quad P_H=\left[\matrix{I& 0\cr -B^T & 0\cr}\right]
$$
and 
$$
P^{V}=GP_VG^{-1}= \left[\matrix{0& B\cr 0 & I\cr}\right] 
\quad P^H=GP_HG^{-1}=\left[\matrix{I& -B\cr 0 & 0\cr}\right]
$$

Notice that the vertical subspace of $T_{\ss,n}N\SS$ is the span of $\PA/\PA y_1,\ldots,\PA/\PA y_m$ and the horizontal
subspace of $T^*_{\ss,n}N\SS$ is the span of $dx_1,\ldots,dx_n$. The map $d\pi_{\ss,n}:T_{\ss,n}N\SS\rarr T_{\ss}\SS$
sends $\PA/\PA x_i\in T_{\ss,n}N\SS$ to $\PA/\PA x_i\in T_{\ss}\SS$ and sends $\PA/\PA y_i\in T_{\ss,n}N\SS$
to $0$. From this it follows that  $J=d\pi_{\ss,n}^{*-1}$, defined on the horizontal subspace of $T^*_{\ss,n}N\SS$
sends $dx_i\in T^*_{\ss,n}N\SS$ to $dx_i\in T^*_{\ss}\SS$. 
If $(\ss,n,\xi,\eta)$ has co-ordinates $(x,y,p,r)$ then $\xi$ has co-ordinates
$$
P^H(x,y)\left[\matrix{p\cr r\cr}\right]=\left[\matrix{p-B(x,y)r\cr 0\cr}\right]
$$
so that $J\xi$ has co-ordinates
$$
p-B(x,y)r.
$$


We now compute the expressions for $H_\lambda$, $H_B$ and $H_O$ in local co-ordinates. 
We will abuse notation and use the same letters to denote functions on $T^*N\SS$ and 
their co-ordinate expressions.
Suppose that the co-ordinates of 
$(\ss,n,\xi,\eta)$ are $(x,y,p,r)$. Since
\be{vertmat}
G^{-1}P^V = P^{VT}G^{-1}P^V = \left[\matrix{0&0\cr 0&I\cr}\right]
\ee
we have that
\be{etanorm}
\jap{\eta,\eta} = \left\langle P^V\left[\matrix{p\cr r}\right],G^{-1}P^V\left[\matrix{p\cr r}\right]\right\rangle
=\jap{r,r}
\ee
Here, and in what follows, inner products involving co-ordinate vectors always refer to Euclidean inner products.
For example, $\jap{r,r} = \sum_{i=1}^m r_i^2$. For the horizontal vectors, we have
$$
\left[\matrix{I&-B\cr 0&I\cr}\right]P^H = P^H
$$
so that
\be{horiz}\eqalign{
\jap{\xi,\xi} &= \left\langle P^H\left[\matrix{p\cr r}\right],G^{-1}P^H\left[\matrix{p\cr r}\right]\right\rangle\cr
&=\jap{(p-Br),(G_\SS+C)^{-1}(p-Br)}\cr
}\ee
Therefore the local co-ordinate expression for $H_\lambda$ is
$$
H_\lambda(x,y,p,r) = {{1}\over{2}}\jap{(p-Br),(G_\SS+C)^{-1}(p-Br)}
+{{1}\over{2}}\jap{r,r} + {{\lambda^4}\over{2}}\jap{y,A(x) y} + V(x,y)
$$
Here $C=C(x,y)$ and $B=B(x,y)$ are the matrices appearing in the expression for the metric $G$,
$A(x)$ is the matrix for $A(\ss)$ in the basis given by the orthonormal frame $n_1,\ldots n_m$ used to define the
co-ordinate system and $V(x,y) = V\big(\ss(x) + \sum y_kn_k(\ss(x))\big)$. Similarly
\be{HB}
H_B(x,y,p,r) = {{1}\over{2}}\jap{(p-Br),G_\SS^{-1}(p-Br)}+ V(x,0)
\ee
where $B=B(x,y)$ and $G_\SS=G_\SS(x)$.
Finally
\be{HO}
H_O(x,y,p,r) = {{1}\over{2}}\jap{r,r} + {{1}\over{2}}\jap{y,A(x) y}
\ee


The expressions for $H_O$ and $I_\alpha$ simplify if we can choose the vectors in the local orthonormal frame to be eigenvectors
of $A(\ss)$. This is always possible if there are no eigenvalue crossings. When, in addition, the eigenvalues $\omega^2_\alpha(\ss)$ do not
depend on $\ss$ there are further simplifications. In what follows we will assume that there are $m_0$ distinct constant eigenvalues
$\omega^2_\alpha$ for  $\alpha = 1,\ldots,m_0$, where $\omega^2_\alpha$ has multiplicity $k_\alpha$. We will assume that the local
orthonormal frame used to the define the co-ordinate system 
consists of eigenvectors for $A(\ss)$. We label them $n_{\alpha,j}$, where $\alpha = 1,\ldots m_0$ and $j=1,\ldots,k_\alpha$
where for each $\alpha$, $n_{\alpha,j}$ is an eigenvector with eigenvalue $\omega^2_\alpha$. This means that
the co-ordinates $y$ and $r$ now also acquire a double labelling. 

First of all we have
$$
H_O(x,y,p,r) = {{1}\over{2}}\jap{r,r} +\half\sum_{\alpha}\omega_\alpha^2\sum_{j} y_{\alpha,j}^2
$$
If the co-ordinates of 
$(\ss,n,\xi,\eta)$ are $(x,y,p,r)$, then
$$
\jap{n,P_\alpha n} = \sum_{j} y_{\alpha,j}^2
$$
The vertical cotangent vector $\eta$ has co-ordinates $P^V\left[\matrix{p\cr r}\right]$. The corresponding tangent vector
has co-ordinates $G^{-1}P^V\left[\matrix{p\cr r}\right]$ which equals $\left[\matrix{0\cr r}\right]$, by \rf{vertmat}.
Now the projection $P_\alpha$, acting on tangent vectors, just picks off the basis vectors $\PA/\PA y_{\alpha, j}$, i.e.,
$P_\alpha\PA/\PA y_{\beta, j}= \delta_{\beta,\alpha} \PA/\PA y_{\beta, j}$. Thus
$$
\jap{\eta,P_\alpha\eta} = \sum_{j} r_{\alpha,j}^2
$$
Therefore
$$
I_\alpha(x,y,p,r) = {{1}\over{2\omega_\alpha}}\sum_{j} r_{\aj}^2
+{{\omega_\alpha}\over{2}}\sum_{j} y_{\alpha,j}^2
$$
Notice that in this situation, where the vectors in the local orthonormal frame are eigenvectors
of $A(\ss)$, neither $H_O$ nor $I_\alpha$ depend on $x$ or $p$.

Now we introduce local action-angle co-ordinates. 
In analogy with creation and destruction operators in quantum mechanics, we define
the complex quantities
$$
a_{\alpha,j} = {{y_{\alpha,j}\omega_\alpha + ir_{\alpha,j}}\over{\sqrt{2\omega_\alpha}}},
$$
so that
$$\eqalign{
y_{\alpha,j} &= {{1}\over{\sqrt{2\omega_\alpha}}}(a_{\alpha,j} + a_{\alpha,j}^*)\cr
r_{\alpha,j} &= -i\sqrt{{{\omega_\alpha}\over{2}}}(a_{\alpha,j} - a_{\alpha,j}^*).\cr
}$$
The action variables $I_{\alpha,j}\in\RR$ and angle variables $\varphi_{\alpha,j}\in S^1$
are then defined by
$$
a_{\alpha,j} = \sqrt{I_{\alpha,j}}e^{i\varphi_{\alpha,j}}
$$
Notice that $\sum_j I_{\alpha,j} = I_\alpha$. The change of co-ordinates from $(x,y,p,r)$ to
$(x,\varphi,p,I)$ is symplectic, since $\sum dr_\aj\wedge dy_\aj = \sum d I_\aj\wedge d\varphi_\aj$.
This makes it easy to compute the flow $\phi_t^{I_\alpha}$ in these co-ordinates. 
Hamilton's equations for the flow are
$$\displaylines{
\dot x_i = 0,\quad \dot p_i = 0,\quad \dot I_\aj = 0\cr
\dot \varphi_{\aj} = \delta_{\beta,\alpha}\cr
}$$
Thus, under the flow $\phi_t^{I_\alpha}$ each $\varphi_\aj$ is translated by
$t$ and all the other variables remain unchanged. This implies that under the
group action $\Phi(\tau)$, with $\tau=(\tau_1,\ldots,\tau_{m_0})$ the quantities
$a_\aj$ evolve as $e^{-i\tau_\alpha}a_\aj$.

We now compute the expression for $H_B$ in action angle co-ordinates.
We find
$$\eqalign{
(Br)_{i} &= \sum_\aj B_{{i},(\aj)}(x,y)r_\aj \cr
&=\sum_{\beta, k,\aj}b_{(\aj),(\beta, k)}^i(x)r_\aj y_{\beta, k}\cr
&=\sum_{\beta, k,\aj}{{b_{(\aj),(\beta, k)}^i(x)}\over{2}}(a_\aj-a_\aj^*)(a_{\beta, k}+a_{\beta, k}^*)\sqrt{{{\omega_\alpha}\over{\omega_\beta}}}\cr
}$$
Here $b_{(\aj),(\beta, k)}^i(x)=b_{(\aj),(\beta, k)}[\ss_i(x)]$ is the antisymmetric matrix given by \rf{connform}. The expression for $H_B$ is now obtained by substituting this formula for $Br$ into \rf{HB}, which we may rewrite as
$$
H_B(x,p,\varphi,I) = \half\sum_{i,l}p_i g^{i,l}p_l
-\sum_{i,l}(Br)_i g^{i,l}p_l
+\half\sum_{i,l}(Br)_i g^{i,l}(Br)_l
+V(x,0)
$$
Here $g^{i,l}=g^{i,l}(x)$ are the matrix elements of $G_\SS^{-1}(x)$.
To obtain the expression for $H_B\circ\Phi(\tau)$ we simply replace each occurrence of $a_\aj$ in the formula above
with $e^{i\tau_\alpha}a_\aj$. Since $H_B$ contains only constant, quadratic and quartic terms in $a_\aj, a_\aj^*$,
we see that the Fourier expansion of $H_B\circ\Phi(\tau)$ has finitely many terms, since the $\nu=(\nu_1,\ldots,\nu_{m_0})$'s that appear
have $\sum_\alpha |\nu_\alpha| \in \{0,2, 4\}$.

\endsection


==> coords2.tex <==
\beginsection
\shd{More co-ordinate expressions}

In this section we give the co-ordinate expressions that will be needed in our proofs
of the quantum theorems.

We begin by defining the second fundamental form, the Weingarten maps and the mean and scalar
curvatures. Let $X$ and $Y$ be two vector fields tangent to $\SS$. Since the Lie bracket $[X,Y]=dY[X]-dX[Y]$ is tangent to $\SS$ we find that
$$
I\hskip -2ptI(X,Y) = P^NdX[Y] = P^NdY[X]+P^N[X,Y]=P^NdY[X]
$$
is symmetric in $X$ and $Y$. Here $P^N$ denotes the projection onto the normal space. By definition, $I\hskip -2ptI(X,Y)$ is the second fundamental form.
Given an orthonormal frame $n_1(\ss),\ldots,n_m(\ss)$ for the normal bundle, 
we have
$$
I\hskip -2ptI(X,Y) = \sum_k\jap{X,S_k Y}n_k
$$
for a collection of symmetric linear transformations $S_k$ on the tangent space. These are called the Weingarten maps.
Clearly $\jap{X,S_k Y}=\jap{n_k,dX[Y]}$. But, by differentiating $\jap{n_k,X}=0$, we obtain $\jap{dn_k[Y],X}+\jap{n_k,dX[Y]}=0$, so
that the Weingarten maps can also be written as
$S_k=-P^T dn_k$. Here $P^T$ denotes the orthogonal projection onto the tangent space. 

The mean curvature vector is given by
\be{meancurv}
h={{1}\over{n}}\sum_{k=1}^m \tr (S_k)n_k
\ee
while the scalar curvature is
\be{scalcurv}
s={{1}\over{n(n-1)}}\sum_{k=1}^m ((\tr(S_k))^2-\tr (S_k^2))
\ee

Recall that the local expression $G(x,y)$ for the pulled back metric on $N\SS$ has the block form \rf{Gblock}.
Initially, $G(x,y)$ is only defined for $\|y\| < \delta$. In our theorem, we wish to extend this metric
to a complete Riemannian metric on all of $N\SS$. One way to achieve this is to join the induced metric for small $|y|$ to the
metric $\jap{\cdot,\cdot}_1$ given by \rf{newmetric} for large $|y|$. Since the matrix for the metric $\jap{\cdot,\cdot}_1$
is
$$
\left[\matrix{I&B\cr 0&I\cr}\right]\left[\matrix{G_\SS&0\cr 0&I\cr}\right]\left[\matrix{I&B\cr 0&I\cr}\right]^T
$$
the resulting metric on all of $N\SS$ would have the  matrix
$$
G(x,y) = \left[\matrix{I&B\cr 0&I\cr}\right]\left[\matrix{G_\SS + \chi C&0\cr 0&I\cr}\right]\left[\matrix{I&B\cr 0&I\cr}\right]^T
$$
where $\chi=\chi(|y|)$ is a cutoff function that equals $1$ for $|y| < \epsilon$ and $0$ for $|y|>\delta$. With this special form of
the extended metric the local co-ordinate expression below remain true on all of $N\SS$ if $C$ is replaced by $\chi C$. However,
this special form of the extension is not required for our theorems.

Let $g(x,y)=\det(G(x,y))=\det(G_\SS+C)$. Define
$$
D_x = \left[\matrix{D_{x_1}\cr\vdots\cr D_{x_n}}\right], \quad
D_y = \left[\matrix{D_{y_1}\cr\vdots\cr D_{y_m}}\right]
$$
The local co-ordinate expression for the operator $H_\lambda = -\half\L + V(\ss,n) + \lambda^4W(\ss,n)$ in the region $|y|<\delta$ is
$$\eqalign{
H_\lambda &= 
-\half g^{-1/2}\left[\matrix{D_x-BD_y\cr D_y}\right]^T g^{1/2}
\left[\matrix{(G_\SS+C)^{-1}&0\cr 0&I\cr}\right]
\left[\matrix{D_x-BD_y\cr D_y}\right] + V(x,y) + {{\lambda^4}\over{2}}\jap{y,A(x) y}\cr
&=-\half g^{-1/2}\Big(
(D_x-BD_y)^T g^{1/2}(G_\SS+C)^{-1}(D_x-BD_y) + D_y^Tg^{1/2}D_y
\Big)\cr
&\hskip 10.4cm + V(x,y) + {{\lambda^4}\over{2}}\jap{y,A(x) y}\cr
}$$

Local expressions for the densities on $N\SS$ are
$$\eqalign{
d{\rm vol} &= \sqrt{g(x,y)}|d^n x| |d^m y|\cr
d{\rm vol}_\lambda &= \sqrt{g(x,y/\lambda)}|d^n x| |d^m y|\cr
d{\rm vol}_{N\SS} &= \sqrt{g(x,0)}|d^n x| |d^m y| = \sqrt{g_\SS(x)}|d^n x| |d^m y|\cr
}$$
where $g_\SS(x) = \det(G_\SS(x))$. Thus the multiplication operator $M_\lambda$ appearing in \rf{unitary}
 is multiplication by $f_\lambda^{-1/4}$ where
$$
f_\lambda(x,y) = {{g(x,y/\lambda)}\over{g_\SS(x)}}.
$$

We may now compute the local expression for $L_\lambda$. Conjugation by $D_\lambda$ results in
every multiplication by a (possibly matrix valued) function $F(x,y)$ being replaced by multiplication by $F(x,y/\lambda)$, and
every $D_y$ being replaced by $\lambda D_y$. Conjugation by $M_\lambda$ simply puts a multiplication
by $f_\lambda^{-1/4}$ to the right of the operator, and a multiplication
by $f_\lambda^{1/4}$ to the left. 
In a co-ordinate system for a domain in $N\SS$ of the form $\{(\ss,n):\ss\in\UU, n\in N\SS_\ss\}$
let $D=\left[\matrix{D_x\cr D_y\cr}\right]$ and $G_\lambda(x,y)$ be the scaled and extended metric taking into account
the scaling of $D_y$ as well as $y$. In other words
\be{seG}
G_\lambda(x,y) = \left[\matrix{I&0\cr 0&\lambda I}\right]G(x,y/\lambda)\left[\matrix{I&0\cr 0&\lambda I}\right].
\ee
Then
\be{preira7.4}\eqalign{
L_\lambda &= -\half f_\lambda^{1/4}g(x,y/\lambda)^{-1/2} D^T g(x,y/\lambda)^{1/2} G_\lambda^{-1} Df_\lambda^{-1/4} +  V(x,y/\lambda) + {{\lambda^2}\over{2}}\jap{y,A(x)y}\cr
&= -\half g_\SS^{-1/2} f_\lambda^{-1/4}D^Tf_\lambda^{1/4}g_\SS^{1/2}G_\lambda^{-1}f_\lambda^{1/4}Df_\lambda^{-1/4} +  V(x,y/\lambda) + {{\lambda^2}\over{2}}\jap{y,A(x)y}\cr
}\ee
Thus in the region where $\|y\| < \delta\lambda$ we may use the explicit form of the metric to obtain
\be{Llexpr}\eqalign{
L_\lambda 
&= -\half f_\lambda^{-1/4}g_\SS^{-1/2}
\left[\matrix{D_x-BD_y\cr D_y}\right]^T g_\SS^{1/2}f_\lambda^{1/2}
\left[\matrix{(G_\SS+C_\lambda)^{-1}&0\cr 0&\lambda^2I\cr}\right]
\left[\matrix{D_x-BD_y\cr D_y}\right]f_\lambda^{-1/4}\cr
&\hskip 2cm + V(x,y/\lambda) + {{\lambda^2}\over{2}}\jap{y,A(x)y},\cr
}\ee
where $C_\lambda(x,y) = C(x,y/\lambda)$. Note that formally putting $f_\lambda=1$ above, and replacing $C_\lambda$ by $0$,
 we obtain for the first line of \rf{Llexpr}
$$
-\half g_\SS^{-1/2}\left[\matrix{D_x\cr D_y\cr}\right]^T
\left[\matrix{I&-B\cr0&I\cr}\right]^Tg_\SS^{1/2}\left[\matrix{G_\SS^{-1}&0\cr 0&\lambda^{2}I\cr}\right]\left[\matrix{I&-B\cr0&I\cr}\right]\left[\matrix{D_x\cr D_y\cr}\right]
$$
which is the Laplace-Beltrami operator for the metric which in local co-ordinates is
$$
\left[\matrix{I&B\cr0&I\cr}\right]\left[\matrix{G_\SS&0\cr 0&\lambda^{-2}I\cr}\right]\left[\matrix{I&B\cr0&I\cr}\right]^T.
$$
This is easily seen to be the matrix for the metric \rf{newmetric}. This explains part of the origin of the $H_B+\lambda^2H_O$. A more
complete analysis (to which we now turn) is necessary to understand the origin of the term $K(\ss)$.

Before beginning this, note that the local expressions for
$H_B$ and $H_O$ are given by
\be{QHB}
H_B = \half (D_x - B(x,y)D_y)^*  G_\SS^{-1}(D_x - B(x,y)D_y) + K(x) + V(x,0)
\ee
and
\be{QHO}
H_0 = \half D_y^*D_y + \half\jap{y,A(x)y}
\ee
Here $D_x^*$ and $D_y^*$ denote the formal adjoints with respect to $d{\rm vol}_{N\SS}$ given by
$D_x^* = -g_\SS^{-1/2}D_x^T g_\SS^{1/2}$, $D_y^* = -g_\SS^{-1/2}D_y^T g_\SS^{1/2}=-D_y^T$ and
$B^*=g_\SS^{-1/2}B^T g_\SS^{1/2}=B^T$.

We now wish to perform a large $\lambda$ expansion of $L_\lambda$. To state the error estimates
precisely, we introduce the notation $E_k$ to denote a smooth function of $x$ and $y$
that vanishes to $k$th order at $y=0$, evaluated at $(x,y/\lambda)$. Roughly speaking,
$E_k$ behaves like $(y/\lambda)^k$ for small $y/\lambda$. 
The effect of differentiating such an error term is given by
$$\eqalign{
{{\PA E_k}\over{\PA x_i}} &= E_k\cr
{{\PA E_k}\over{\PA y_i}} &= \cases{
\lambda^{-1}E_{k-1} & if $k\ge 1$\cr 
\lambda^{-1}E_{0} & if $k=0$\cr}\cr
}$$

In our theorems we will always assume that the eigenvalues $\omega_j^2$ of $A(\ss)$ are constant. If we choose the
orthonormal frame in the definition of our co-ordinates to consist of eigenvectors of $A(\ss)$ then
$\jap{n,A(\ss)n} = \sum_j\omega^2_jy_j^2$. We will make this substitution without further comment below.

\beginlemmalabel{Lexpression} In the region where $\|y\| < \delta\lambda$, the local expression for
$L_\lambda$ can be written
$$
L_\lambda = H_B + \lambda^2 H_0 
+ (D_x - BD_y)^* E_1(D_x-BD_y)+ E_1.
$$
\endlemma

\beginproof
In a co-ordinate system for a domain in $N\SS$ of the form $\{(\ss,n):\ss\in\UU, n\in N\SS_\ss\}$
let $D=\left[\matrix{D_x\cr D_y\cr}\right]$ and $G_\lambda(x,y)$ be given by \rf{seG}. 
Setting $k_\lambda = (1/4)\ln f_\lambda$, we may write \rf{preira7.4} as
\be{ira7.4}
L_\lambda = \half (D-\PA k_\lambda)^*G_\lambda^{-1}(D-\PA k_\lambda) + V(x,y/\lambda)  + {{\lambda^2}\over{2}}\sum_j\omega^2_jy_j^2
\ee
where $\PA k_\lambda = \left[\matrix{\PA_x k_\lambda\cr \PA_y k_\lambda\cr }\right]$, $\PA k_\lambda^* = (\PA k_\lambda)^T$, and
$D^* = -g_\SS^{-1/2} D^T g_\SS^{1/2}$. We further expand \rf{ira7.4} to obtain
\be{ira7.5}
L_\lambda = \half D^*G_\lambda^{-1}D + \half \PA k_\lambda^*G_\lambda^{-1}\PA k_\lambda + 
\half \sum_{i,j} g_\SS^{-1/2} \PA_i\left( g_\SS^{1/2}\left(G_\lambda^{-1}\right)_{i,j}\PA_jk_\lambda\right)
+ V(x,y/\lambda) + {{\lambda^2}\over{2}}\sum_j\omega^2_jy_j^2
\ee
If $\|y\|<\lambda\delta$ then
\be{ira7.6}
G_\lambda^{-1}(x,y) = \left[\matrix{I&-B(x,y)\cr 0&I\cr}\right]^T
\left[\matrix{\left(G_\SS(x) + C(x,y/\lambda)\right)^{-1}&0\cr 0& \lambda^2 I\cr}\right]
\left[\matrix{I&-B(x,y)\cr 0&I\cr}\right]
\ee
so that in this region we obtain
$$\eqalign{
L_\lambda &= \half (D_x-BD_y)^*G_\SS(x)^{-1}(D_x-BD_y) + {{\lambda^2}\over{2}} D_y^*D_y\cr
&\quad+(D_x-BD_y)^*E_1(D_x-BD_y) + E_1 + {{\lambda^2}\over{2}}\sum_i\left( \PA_{y_i}^2k_\lambda + (\PA_{y_i}k_\lambda)^2\right)\cr
&\quad+V(x,y/\lambda) + {{\lambda^2}\over{2}}\sum_j\omega^2_jy_j^2\cr
&=H_B+\lambda^2H_O + (D_x-BD_y)^*E_1(D_x-BD_y) + E_1\cr
&\quad+{{\lambda^2}\over{2}}\sum_i\left( \PA_{y_i}^2k_\lambda + (\PA_{y_i}k_\lambda)^2\right) -K(x)\cr
}$$
Here we used $(\PA_x-B\PA_y)E_k = E_k$ and $\PA k_\lambda = \left[\matrix{E_1\cr \lambda^{-1} E_0\cr}\right]$, so that
$(\PA_x-B\PA_y)k_\lambda = E_1$.

The lemma will follow if we can show
\be{ira7.7}
{{\lambda^2}\over{2}}\sum_i\left( \PA_{y_i}^2k_\lambda + (\PA_{y_i}k_\lambda)^2\right) =K(x) + E_1
\ee

This requires a more careful expansion of $f_\lambda$. The first step is to uncover the
geometrical meaning of the term $G_\SS(x) + C(x,y)$ occurring in the expression \rf{Gblock} for the metric.
Note that
$$
\jap{dn_k[\ss_i],\ss_j} = -\jap{S_k\ss_i,\ss_j} = -\jap{\ss_i,S_k\ss_j} = \jap{\ss_i,dn_k[\ss_j]} 
$$
and that
$$
M_k = G_\SS^{-1}[\jap{\ss_i,S_k \ss_j}]
$$
is the matrix for the Weingarten map $S_k$ in the basis $\ss_1,\ldots,\ss_n$. 
Let $S$ be the symmetric operator defined by
$\jap{n, I\hskip -2ptI(X,Y)} = \jap{X,S Y}$. Then $S = \sum_k y_k S_k$, and 
the matrix for $S$ in the basis $\ss_1,\ldots,\ss_n$ is
$$
M= M(x,y) = \sum_k y_k M_k(x)
$$
A short calculation shows
\be{GplusC}
G_\SS + C = G_\SS(I-M)^2
\ee
Given the block form \rf{Gblock} of $G$ and \rf{GplusC},  we obtain
$$\eqalign{
f_\lambda &= g_\lambda/g_\SS = \det(G(x,y/\lambda)/\det(G_\SS(x))\cr 
&= \det(G_\SS(x)(I-\lambda^{-1}M(x,y))^2)/\det(G_\SS(x))\cr
&=\det(I-\lambda^{-1}M(x,y))^2.\cr
}$$
Thus
$$\eqalign{
k_\lambda &= \half\ln(f_\lambda^{1/2}) = \half \ln\det(I-\lambda^{-1}M)\cr
&=\half {\rm tr}\ln(I-\lambda^{-1}M)\cr
&=-\half \lambda^{-1}{\rm tr}(M) - {{1}\over{4}}\lambda^{-2}{\rm tr}(M^2) + E_3\cr
&=-\half \lambda^{-1}\sum_k y_k {\rm tr}(S_k)
- {{1}\over{4}}\lambda^{-2}\sum_{k,l}y_ky_l{\rm tr}(S_kS_l) + E_3\cr
}$$
This implies that
$$
\PA _{y_i} k_\lambda = -\half \lambda^{-1}{\rm tr}(S_i)+ \lambda^{-2}E_1+ \lambda^{-1}E_2
$$
and
$$
(\PA _{y_i})^2 k_\lambda = -\half \lambda^{-2}{\rm tr}(S_i^2)+ \lambda^{-2}E_1.
$$
Thus
$$\eqalign{
{{\lambda^2}\over{2}}\sum_i\left( \PA_{y_i}^2k_\lambda + (\PA_{y_i}k_\lambda)^2\right)
&=-{{1}\over{4}}{\rm tr}(S_i^2) + {{1}\over{8}}({\rm tr}(S_i))^2+ E_1\cr
&={{1}\over{4}}\left(({\rm tr}(S_i))^2-{\rm tr}(S_i^2)\right)  -{{1}\over{8}}({\rm tr}(S_i))^2+ E_1\cr
&={{n(n-1)}\over{4}} s - {{n^2}\over{8}}\|h\|^2 + E_1\cr
}$$
Thus proves \rf{ira7.7} and completes the proof
\endproof

We conclude this section by discussing the expression for $\HBbar$ in local co-ordinates. We may define local annihilation and creation operators, using the co-ordinates $y_{\alpha,j}$
defined in Section 5, as
$$\eqalign{
a_{\alpha,j} &= {{1}\over{\sqrt{2\omega_\alpha}}}(\omega_{\aj}y_\aj + D_{y_\aj})\cr
a_{\alpha,j}^* &= {{1}\over{\sqrt{2\omega_\alpha}}}(\omega_{\aj}y_\aj - D_{y_\aj})\cr
}$$
Then we find
$$\eqalign{
I_\alpha &= \sum_j\left( -{{1}\over{2\omega_\alpha}}D_{y_\aj}^2 + {{\omega_\alpha}\over{2}}y_\aj^2\right)\cr
&= \sum_j\left( a_\aj^* a_\aj + \half\right)\cr
}$$

We may also write $H_B$ in terms of the annihilation and creation operators. We begin with
$$
(B(x,y)D_y)_i = \sum_{\aj,\bk}b^i_{\aj, \bk} D_{y_\aj}y_\bk.
$$
Notice that the order of $D_{y_\aj}$ and $y_\bk$ is irrelevant here, since $b^i$ is antisymmetric in $(\aj)$ and $(\bk)$.
Then we can use
$$\eqalign{
D_{y_\aj} &= \sqrt{{{\omega_\alpha}\over{2}}}\left( a_\aj - a^*_\aj\right)\cr
y_\bk &= \sqrt{{{1}\over{2\omega_\alpha}}}\left( a_\bk + a^*_\bk\right)\cr
}$$
and substitute the resulting expression in \rf{QHB}. The resulting formula expresses $H_B$ as a finite sum of terms
involving product of $0$, $2$ or $4$ annihilation or creation operators. The identities
\be{aconj}
e^{itH_O}a_\aj e^{-itH_O} = e^{-it\omega_\alpha}a_\aj\quad \quad
e^{itH_O}a^*_\aj e^{-itH_O} = e^{it\omega_\alpha}a^*_\aj
\ee
lead to a finite sum
$$
e^{itH_O}H_Be^{-itH_O} = \sum_{\nu\in\ZZ^{m_0}}e^{it\jap{\nu,\omega}}F_\nu
$$
that defines the differential operators $F_\nu$.

\beginlemma
For $\varphi\in C_0^{\infty}(N\SS)$, $e^{-itH_O}\varphi \in {\cal D}(H_B)$ and
\be{HBexpansion}
e^{itH_O}H_Be^{-itH_O}\varphi = \sum_{\nu\in\ZZ^{m_0}} e^{it\jap{\nu,\omega}}F_\nu\varphi
$$
where the operators $F_\nu$ are defined by the sum above. 
\endlemma
\beginproof
It suffices to prove this for $\varphi\in C_0^\infty$ supported in a single co-ordinate patch, since a
general $\varphi\in C_0^\infty$ can be written as a sum of such functions. Introducing our usual 
local co-ordinates $x$ and $y$, we find that $e^{-itH_O}$ is simply a harmonic oscillator time evolution
in the $y$ variables. Hence $e^{-itH_O}\varphi$ is in Schwartz space. This implies that $e^{-itH_O}\varphi \in {\cal D}(H_B)$, and
that the expansion
of $H_B$ into a sum of terms involving products of $a_\aj$ and $a^*_\aj$ is valid when applied to $e^{-itH_O}\varphi$. 
To complete the proof, it remains to show that the identities \rf{aconj} hold when applied to a function $\varphi$ in Schwartz space.
This follows from
$$\eqalign{
{{d}\over{dt}}e^{itH_O} a_\aj e^{-itH_O}\varphi &= ie^{itH_O} [H_O,a_\aj] e^{-itH_O}\varphi\cr
&= i\omega_\alpha e^{itH_O} [a^*_\aj a_\aj, a_\aj] e^{-itH_O}\varphi\cr
&= i\omega_\alpha e^{itH_O} [a^*_\aj,a_\aj]a_\aj e^{-itH_O}\varphi\cr
&=-i\omega_\alpha e^{itH_O} a_\aj e^{-itH_O}\varphi.\cr
}$$
\endproof
\endsection


==> intro.tex <==
\beginsection
\shd{Introduction}

Consider a system of non-relativistic particles in 
a Euclidean configuration space $\RR^{n+m}$ whose motion is governed
by the Hamiltonian
\be{hamorig}
H = \half\jap{p,p} + V(x).
\ee
We are interested 
in the motion of
these particles when their positions are constrained to lie on
some $n$-dimensional submanifold $\SS\subset\RR^{n+m}$. In both classical and quantum
mechanics there are accepted notions about what 
the constrained motion should be:

In classical mechanics, the Hamiltonian for the constrained motion is assumed to have
the form \rf{hamorig}, but whereas  $p$ and $x$ originally denoted variables on
the phase space $T^*\RR^{n+m}=\RR^{n+m}\times\RR^{n+m}$, they now are variables
on the cotangent bundle $T^*\SS$. The inner product $\jap{p,p}$ is now computed using the metric that $\SS$ inherits from $\RR^{n+m}$, and $V$ now denotes the restriction of $V$ to $\SS$.

In quantum mechanics, $\jap{p,p}$ is interpreted to mean $-\L$, where $\L$ is the Laplace operator, and $V(x)$ is
the operator of multiplication by $V$. 
For unconstrained motion $\L$ is the Euclidean Laplacian on $\RR^{n+m}$,
and the Hamiltonian acts in $L^2(\RR^{n+m})$. For constrained motion, 
the Laplace operator for $\SS$ with the inherited metric is used, and
the Hilbert space is $L^2(\SS, d{\rm vol})$. 

In both cases the description of the constrained motion is
intrinsic: it depends only on the Riemannian structure that
$\SS$ inherits from
$\RR^{n+m}$, but not on other details of the imbedding.

Of course, a constrained system of particles is an idealization. 
Instead of particles moving exactly on $\SS$, one might imagine there is a 
strong force pushing the particles onto the submanifold. The motion of the
particles would then be governed by the Hamiltonian
\be{hamlambda}
H_\lambda =  \half\jap{p,p} + V(x) + \lambda^4 W(x)
\ee
where $W$ is a positive potential vanishing exactly on $\SS$ and $\lambda$
is large. (The fourth power is just for notational convenience later on.) Does the motion described by $H_\lambda$ converge to the intrinsic
constrained motion as $\lambda$ tends to infinity? Surprisingly, the answer
to this question depends on exactly how it is asked, and is often no.

A situation in classical mechanics where the answer is yes is described by
Rubin and Ungar [RU]. An initial position on $\SS$ and an initial velocity
tangent to $\SS$ are fixed. Then, for a sequence of $\lambda$'s tending to
infinity, the subsequent motions under $H_\lambda$ are computed. As
$\lambda$ becomes large, these motions converge to the intrinsic
constrained motion on $\SS$. This result is widely known, since it appears
in Arnold's book [A1] on classical mechanics. However, from the physical
point of view, it is neither completely natural to require that the initial
position lies exactly on $\SS$, nor that the initial velocity be exactly tangent. 
Rubin and Ungar also consider what happens if the initial velocity has
a  component in the direction normal to $\SS$. In this case, the motion in
the normal direction is highly oscillatory, and there is an extra potential
term, depending on the initial condition,  in the Hamiltonian for the
limiting motion on $\SS$.  In their proof, $\SS$ is assumed to have co-dimension one.
A more complete result is given by Takens [T].
Here the initial conditions are allowed to depend on $\lambda$ in such a
way that the initial position converges to a point on $\SS$ and the initial
energy remains bounded. (We will give precise assumptions below.) Once
again, the limiting motion on $\SS$ is governed by a Hamiltonian with an
additional potential. Takens noticed that a non-resonance condition on the
eigenvalues of the Hessian of the constraining potential $W$ along $\SS$ is
required to prove convergence. He also gave an example showing that if the
Hessian of $W$ has an eigenvalue crossing, so that the non-resonance condition is
violated, then there may not be a
good notion of limiting motion on $\SS$. In his example, he constructs two sequences
of orbits, each one converging to an  orbit on $\SS$. These
limiting orbits are identical until they hit the point on $\SS$ where the
eigenvalues cross. After that, they are different. This means there is no
differential equation on $\SS$ governing the limiting motion. For other
discussions of the question of realizing constraints see [A2] and [G]. A modern
survey of the classical mechanical results that emphasizes the systematic
use of weak convergence is given by Bornemann and Sch\"utte [BS].

The quantum case was considered previously by Tolar [T], da Costa [dC1, dC2] and
in the path integral literature (see Anderson and Driver [AD]). 
Related work can also be
found in Helffer and Sj\"ostrand [HS1] [HS2], who obtained WKB expansions for
the ground state, and in Duclos and Exner [DE], Figotin and Kuchment [FK], Schatzman [S]
and Kuchment and Zeng [KZ].
There are really two aspects to the problem of realizing
constraints: a large $\lambda$ expansion followed by an averaging procedure
to deal with highly oscillatory normal motion. Previous work 
in quantum mechanics
concentrated on the first aspect (although a related averaging procedure for classical paths with a vanishingly small random perturbation can be found in [F] and [FW]). Already a formal large $\lambda$ expansion
reveals the interesting feature that the limiting Hamiltonian has an extra
potential term depending on scalar and the mean curvatures.  Since
the mean curvature is not intrinsic, this potential does depend on the
imbedding of $\SS$ in $\RR^{n+m}$. 

It is not completely straightforward to
formulate a theorem in the quantum case. We have chosen a formulation,
modeled on the classical mechanical theorems, tracking a sequence
of orbits with initial positions concentrating on $\SS$ via dilations
in the normal direction. Actually we consider the equivalent problem
of tracking the evolution of a fixed vector governed by the 
Hamiltonian $H_\lambda$ conjugated by  unitary dilations.
In order
to obtain simple limiting asymptotics for the orbit
we must assume that all the eigenvalues of the Hessian of the constraining
potential $W$ are constant on $\SS$. In fact we will assume that $W$ is
exactly quadratic. Our theorems show that for large $\lambda$ the motion
is approximated by the motion generated by an averaged limiting Hamiltonian $\HBbar$, with
superimposed normal oscillations generated by $\lambda^2 H_O$, where $H_O$ is the normal harmonic
oscillator Hamiltonian. The Hamiltonians $\HBbar$ and $H_O$ commute, so the motions are independent.
These theorems do not require any non-resonance conditions on the eigenvalues of the Hessian of $W$.
However, the limiting Hamiltonian $\HBbar$ does not act in $L^2(\SS)$, but in $L^2(N\SS)$ where
$N\SS$ is the normal bundle of $\SS$. 
It is only in certain situations where one can effectively ignore the motion in the normal
directions and obtain a unitary group on $L^2(\SS)$ implementing the dynamics of the
tangential motion. This occurs, for example, if (a) the eigenvalues of the Hessian of $W$ are
all distinct and non-resonant, (b) the normal bundle is trivial, and (c) we confine our attention
to a simultaneous eigenspace of all the number operators for the normal motion. In the general
situation, the dynamics of the additional degrees of freedom in $N\SS$ cannot be factored out, and we
must be content with analysis on $L^2(N\SS)$.

Our formulation of the quantum theorems invites comparison with the
classical mechanical results of Rubin and Ungar [RU] and Takens [T]. 
It turns out that extra potentials that appear
in the two cases are quite different, and there is no obvious connection.
Upon reflection, the reason for this difference is clear. If we have a
sequence of initial quantum states whose position distribution is being
squeezed to lie close to $\SS$, then by the uncertainty principle, the
distribution of initial momenta will be spreading out, and thus the initial
energy will be unbounded. However, the classical mechanical convergence
theorems above all deal with bounded energies. 
The danger in considering unbounded energies is that even if the initial
energy in the tangential mode is bounded, the coupling between tangential 
and normal modes may result in unbounded tangential energy in finite time.
Our assumptions, which allow us to obtain a classical theorem despite the
unbounded energy, are motivated by quantum mechanics. Our results for classical
mechanics with unbounded initial energies are quite similar to our results in quantum mechanics.
 
\bigskip
\centerline{\sl Table of Contents}
\medskip
$$\vbox{\halign{
#\dotfill&\dots#\hfill\cr
1.~Introduction & 1 \cr
2.~Classical mechanics: bounded energy & 4\cr
3.~Classical mechanics: unbounded energy& 7\cr
4.~Quantum mechanics& 12\cr
5.~Co-ordinate expressions& 16\cr
6.~Proofs of theorems in classical mechanics& 20\cr
7.~More co-ordinate expressions& 28\cr
8.~Proofs of theorems in quantum mechanics& 34\cr
}}$$
\bigskip
Section 2 contains a statement of the theorem of Rubin, Ungar and Takens on limiting orbits when the initial energies
remain bounded. In Section 3 we state our expansion and averaging theorems in classical mechanics when the initial energies scale as they do in quantum mechanics. We also describe when the limiting motion can be thought of as a motion on $\SS$.
These classical results are motivated by the parallel results in quantum mechanics, which we present in Section 4. The proofs of the theorems in Sections 3 and 4 are found in Sections 6 and 8 respectively, while Sections 5 and 7 contain background material needed in the proofs.
This paper is an expanded and improved version of the announcement [FH]. 

\endsection


==> quantum.tex <==
\beginsection
\def\dvns{d{\rm vol}_{N\SS}}
\def\dvs{d{\rm vol}_{\SS}}
\shd{Quantum mechanics}

In quantum mechanics, we wish to understand the time evolution
generated by $H_\lambda$ for large $\lambda$, where $H_\lambda$ is the 
Hamiltonian given by \rf{hamlambda} with $\jap{p,p}=-\L$. As in the classical
case, it is convenient to replace the 
original configuration space $\RR^{n+m}$ with 
the normal
bundle $N\SS$. We will show that if the  initial conditions in $L^2(\RR^{n+m})$ 
are supported near $\SS$ then, to a good
approximation for large $\lambda$, the time evolution stays near $\SS$. 
Thus we lose nothing
by inserting Dirichlet boundary conditions on the boundary of the tubular 
neighbourhood of $\SS$, and may transfer our considerations to 
$L^2(N\SS_\delta,d{\rm vol})$, where $d{\rm vol}$ is computed using the
pulled back metric. If we extend the pulled back metric, and make a suitable
definition of $H_\lambda$ in the complement of $N\SS_\delta$, we may remove
the boundary condition. Thus we may assume that that the Hamiltonian 
$H_\lambda$ acts in $L^2(N\SS,d{\rm vol})$.

More precisely, we let $g_{N\SS}$ be any complete smooth Riemannian metric on $N\SS$
that equals the metric induced from the imbedding in the region $\{(\ss,n):\|n\|<\epsilon\}$,
for some $\epsilon < \delta$. For example, such a $g_{N\SS}$ could be obtained by smoothly
joining the induced metric for small $\|n\|$ with the metric $\jap{\cdot,\cdot}_1$ given
by \rf{newmetric} for large $\|n\|$. Let $d\hbox{vol}$ denote the Riemannian density for $g_{N\SS}$.
Let $V(\ss,n)$ be a smooth bounded function on
$N\SS$ such that $V(\ss,n)=V(\ss+n)$ when $\|n\|<\epsilon$. Our goal in this section is
to analyze the time evolution generated by
\be{Hext}
H_\lambda = -\half \L + V(\ss,n) + {{\lambda^4}\over{2}}\jap{n,A(\ss)n}
\ee
acting in $L^2(N\SS,d\hbox{vol})$. Here $\L$ denotes the Laplace-Beltrami operator for $g_{N\SS}$. 
 
We now introduce the group of dilations in the normal directions by defining
$$
(D_\lambda\psi)(\ss,n)=\lambda^{m/2}\psi(\ss,\lambda n).
$$
This is a unitary operator from $L^2(N\SS,d{\rm vol}_\lambda)$ to
$L^2(N\SS,d{\rm vol})$ where $d{\rm vol}_\lambda$ denotes the pulled back
density $d{\rm vol}_\lambda(\ss,n)=d{\rm vol}(\ss,\lambda^{-1}n)$. Since
the spaces $L^2(N\SS,d{\rm vol}_\lambda)$ depend on $\lambda$, 
and we want to
deal with a fixed Hilbert space as $\lambda\rarr\infty$, we perform an an
additional unitary transformation. Let
$$
\dvns = \lim_{\lambda\rarr\infty}d{\rm vol}_\lambda
=\dvs\otimes d{\rm vol}_{\RR^{m}}
$$
Then the quotient of densities $\dvns/d{\rm vol}_\lambda$ is a function
on $N\SS$ and we may define $M_\lambda$ to be the operator of multiplication
by $\sqrt{\dvns/d{\rm vol}_\lambda}$. The operator $M_\lambda$ is unitary
from $L^2(N\SS,\dvns)$ to $L^2(N\SS,d{\rm vol}_\lambda)$. Let
\be{unitary}
U_\lambda = D_\lambda M_\lambda.
\ee
Notice that the support of a family of initial conditions of the form
$U_\lambda\psi$ is being squeezed close to $\SS$ 
as $\lambda\rarr\infty$. We want to consider such a sequence 
of initial conditions. 
Therefore it is natural to
consider the
conjugated Hamiltonian 
$$
L_\lambda = U_\lambda^*H_\lambda U_\lambda,
$$
since the evolution generated by $L_\lambda$ acting on $\psi$ is unitarily
equivalent to the evolution generated by $H_\lambda$ acting on
$U_\lambda\psi$.

As a first step we perform a large $\lambda$ expansion. Formally, this yields
$$
L_\lambda = H_B + \lambda^2 H_O + O(\lambda^{-1})
$$
where $H_O$ is the quantum harmonic oscillator Hamiltonian in the normal
variables, and $H_B$ is quantum version of the corresponding classical
Hamiltonian, except with an additional potential
$$
K = {{n(n-1)}\over{4}} s - {{n^2}\over{8}} \|h\|^2.
$$
Here $s$ is the scalar curvature and $h$ is the mean curvature vector (see equations \rf{scalcurv} and \rf{meancurv}).
Notice that this extra potential does depend on the imbedding of $\SS$ in
$\RR^{n+m}$, since the mean curvature does. The quadratic forms for
$H_O$ and $H_B$ are
\be{QHOqf}
\jap{\psi, H_O\psi} = \int_{N\SS} \half\jap{P^Vd\psi,P^Vd\psi}_{\ss,n} + \half\jap{n,A(\ss)n}|\psi|^2 \dvns
\ee
and
\be{QHBqf}
\jap{\psi, H_B\psi} = \int_{N\SS} \half\jap{JP^Hd\psi,JP^Hd\psi}_\ss + (V(\ss,0) + K(\ss))|\psi|^2 \dvns.
\ee
Local co-ordinate expressions for these operators are given by \rf{QHO} and \rf{QHB} below.
As in the classical case, we can gain additional understanding of these operators by introducing the metric
\rf{newmetric}. Then
$$
H_B + \lambda^2 H_O  = -\half\L_\lambda + {{\lambda^2}\over{2}}\jap{n, A(\ss)n} + V(\ss,0)+K(\ss),
$$
where $\L_\lambda$ is the Laplace-Beltrami operator on $N\SS$ with the metric \rf{newmetric}. 
Note that the volume element $\dvns$ is actually $\lambda^m$ times the usual volume element associated
to this metric (see Section 7).

The operator $H_O$ is explicitly given on $C^2$ functions in its domain by the formula
$$
(H_O\psi)(\ss,n) = \left(-\half \sum_{k=1}^m {{\PA^2}\over{\PA y_k^2}} + \half \jap{n, A(\ss)n}\right)\psi(\ss,\sum_{k=1}^m y_k n_k(\ss)),
$$
where $\{n_k(\ss):k=1\ldots m\}$ is any orthonormal basis for $N\SS$ and $n=\sum_{k=1}^m y_k n_k(\ss)$.

It is easy to show that with the metric \rf{newmetric}, $N\SS$ is complete so that any positive integer power of $H_B + \lambda^2 H_O$ is essentially self-adjoint on $C_0^\infty$ for $\lambda > 0$ [C]. Similarly, because $H_O$ is basically a harmonic oscillator Hamiltonian, it is straightforward
to show that any positive integer power of $H_O$ is essentially self-adjoint on $C_0^\infty$. The operator $H_B$ is more complicated, but also
can be shown to be essentially self-adjoint on $C_0^\infty$. The argument is not difficult and will be omitted. 

\begintheoremlabel{quantum1}
Let $g_{N\SS}$ be a complete smooth Riemannian metric on $N\SS$ that coincides with the induced metric when $\|n\|<\epsilon$,
for some $\epsilon <\delta$, and suppose $V(\ss,n)$ is a bounded smooth extension of $V(\ss+n)$. Let $H_\lambda$ be 
the Hamiltonian given by \rf{Hext}, acting in $L^2(N\SS,d\hbox{\rm vol})$. Assume that $A(\ss)$ varies smoothly, and that the eigenvalues of $\omega_\alpha^2$ of $A(\ss)$ do not
depend on $\ss$.
\par\noindent Let $L_\lambda = U_\lambda^*H_\lambda U_\lambda$
acting in $L^2(N\SS,\dvns)$. Then, for every $\psi\in L^2(N\SS,\dvns)$ and every $T>0$
$$
\lim_{\lambda\rarr\infty} \sup_{0\le t\le T}
\left\|\left(e^{-itL_\lambda}-e^{-it(H_B+\lambda^2H_O)}\right)\psi\right\| = 0
$$
\endtheorem

Just as in the classical case, this theorem provides a satisfactory
description of the motion if $[H_B,H_O]=0$, so that 
$\exp(-it(H_B+\lambda^2H_O))=\exp(-itH_B)\exp(-it\lambda^2H_O)$. As before,
this will happen, for example, if $\SS$ has co-dimension one, or if all the
frequencies $\omega_\alpha$ are equal.

If $\SS$  has co-dimension one, then the normal bundle is trivial. (We are
assuming that $\SS$ is compact.) Then we have $L^2(N\SS,\dvns)=
L^2(\SS,\dvs)\otimes L^2(\RR,dy)$ and $H_B=h_B\otimes I$ for a 
Schr\"odinger operator $h_B$ acting in $L^2(\SS,\dvs)$. Since 
$H_O=I\otimes h_O$ we have that
$\exp(-it(H_B+\lambda^2H_O))=\exp(-ith_B)\otimes\exp(-it\lambda^2 h_O)$.
This can be interpreted as a motion in $L^2(\SS,\dvs)$ with superimposed normal
oscillations.

In the case where the frequencies $\omega_\alpha$ are all equal, the normal
bundle may be non-trivial, and there is not such a simple tensor product
decomposition of $L^2(N\SS,\dvns)$. 
However, for some initial conditions $\psi$ the limiting motion may again be thought of as
taking place in $L^2(\SS,\dvs)$ with superimposed oscillations. For
example, consider the subspace of functions in $L^2(N\SS,\dvns)$ that are
radially symmetric in the fibre variable $n$. This subspace does have a
tensor product decomposition $L^2(\SS,\dvs)\otimes
L^2_{\rm radial}(\RR^m,d^m y)$. It is an invariant subspace for $H_B$.
Furthermore, the restriction of $H_B$ to this subspace has the
form $h_B\otimes I$. Thus, if $\psi_0$ is a radial function in $n$, then
$\exp(-itL_\lambda)\psi_0 = \exp(-ith_B)\otimes\exp(-it\lambda^2 h_O)\psi_0$.
As above, we interpret this as motion in $L^2(\SS,\dvs)$ with superimposed normal
oscillations.

On the other hand, if the normal bundle is non-trivial, it may happen that the limiting motion takes place
on a space of sections of a vector bundle over $\SS$. Instead of giving more
details about the general case, we offer the following illustrative example.
Instead of a normal bundle, consider the M\"obius band $\cal B$ defined by
$\RR\times\RR\,/\sim$, where $(x,y)\sim (x+1,-y)$. This an $O(1)$ bundle
over $S^1$ with fibre $\RR$. An $L^2$ function $\psi$ 
on $\cal B$ can be thought
of as a function on $\RR\times\RR$ satisfying $\psi(x+1,-y)=\psi(x,y)$. If 
we decompose $\psi(x,y)$, for fixed $x$, into odd and even functions of $y$
$$
\psi(x,y) = \psi_{\rm{even}}(x,y) + \psi_{\rm{odd}}(x,y)
$$ 
then $\psi_{\rm{even}}(x+1,y)=\psi_{\rm{even}}(x,y)$
and $\psi_{\rm{odd}}(x+1,y)=-\psi_{\rm{odd}}(x,y)$. 
(Notice that these are eigenfunctions for the left regular representation of
$O(1)$ on $L^2(\RR)$.)
Thus $\psi_{\rm{even}}$
can be thought of as an $L^2(\RR, dy)$ valued function on $S^1$, while
$\psi_{\rm{odd}}$ can be thought of as an 
$L^2(\RR, dy)$ valued section of a
line bundle over $S^1$ (which happens to be $\cal B$ itself). In this
way we obtain the decomposition
$$
L^2({\cal B}) = L^2(S^1,dx)\otimes L^2_{\rm{even}}(\RR, dy) \,\oplus\,
\Gamma(S^1,dx)\otimes L^2_{\rm{odd}}(\RR, dy)
$$
where $\Gamma$ is the space of $L^2$ sections of $\cal B$.

In this example, the bundle is flat, so  $H_B=-D_x^2+V(x)$ and
$H_O=-D_y^2$ acting in $L^2({\cal B},dxdy)$. Let $h_+ = -D_x^2+V(x)$ acting
in $L^2(S^1,dx)$ and $h_-=-D_x^2+V(x)$ acting in $\Gamma(S^1,dx)$. Let
$h_0=-D_y^2$ acting in $L^2(\RR,dy)$, with $L^2_{\rm{even}}(\RR, dy)$ and
$L^2_{\rm{odd}}(\RR, dy)$ as invariant subspaces. Then
$$
e^{-it(H_B+\lambda^2 H_O)}=e^{-ith_+}\otimes e^{-it\lambda^2h_O}
\,\oplus\, e^{-ith_-}\otimes e^{-it\lambda^2h_O}
$$
So if the initial condition  happens to lie in $\Gamma\otimes
L^2_{\rm{odd}}$, then we would think of the limiting motion as taking place
in $\Gamma$, with superimposed oscillations in $L^2_{\rm{odd}}$.

When $H_B$ and $H_O$ do not commute, we perform a quantum version of averaging. Define
$\HBbar$ on $C_0^\infty$ by
\be{QHBbarqf}
\HBbar\psi = \lim_{T\rarr\infty}T^{-1}\int_0^\infty e^{itH_O}H_Be^{-itH_O}\psi\, dt
\ee
It can be shown that $\HBbar$ is essentially self-adjoint.


\begintheoremlabel{quantum2}
Assume that the hypotheses of \thmrf{quantum1} hold. Let $H_O$, $H_B$, and $\HBbar$ be the Hamiltonians defined by
\rf{QHOqf}, \rf{QHBqf} and \rf{QHBbarqf}. Then, for every $\psi\in L^2(N\SS,\dvns)$ and every $T>0$
$$
\lim_{\lambda\rarr\infty}\sup_{0\le t\le T} \left\|\left(e^{-it(H_B+\lambda^2H_O)} - e^{-it\lambda^2H_O}e^{-it\HBbar}\right)\psi\right\| = 0
$$
\endtheorem

The proof that this limit defining $\HBbar$ exists parallels the discussion in classical mechanics. Suppose that there are $m_0$
distinct eigenvalues $\omega_1^2,\ldots,\omega_{m_0}^2$. For each $\alpha = 1,\ldots,m_0$ define the operators
$I_\alpha$ via the quadratic forms
$$
\jap{\psi,I_\alpha\psi} = \int_{N\SS}\left({{1}\over{2\omega_\alpha}}\jap{P^Vd\psi, P_\alpha P^Vd\psi} + {{\omega_\alpha}\over{2}}\jap{n,P_\alpha n}|\psi|^2\right)\dvns
$$
These operators all commute and satisfy
$$
\sum_\alpha \omega_\alpha I_\alpha = H_O.
$$
An expression for $I_\alpha$ in terms of local creation and annihilation operators will be given near the end of Section 7. In that
section we will show that
$e^{i\tau I_\alpha}H_Be^{-i\tau I_\alpha}$ is periodic in $\tau$ with period $2\pi$. Thus if we conjugate $H_B$ with 
$e^{i\sum \tau_\alpha I_\alpha}$, the resulting operator is defined on the torus $T^{m_0}$ and has a Fourier expansion
$$
e^{i\sum\tau_\alpha I_\alpha}H_Be^{-i\sum\tau_\alpha I_\alpha} = \sum_{\nu\in\ZZ^{m_0}}e^{i\jap{\nu,\tau}}F_\nu
$$
Here $\tau=(\tau_1,\ldots,\tau_{m_0})$ and the coefficients $F_\nu$ are differential operators. 
As in the classical case, the sum is finite. Thus
$$
e^{itH_O}H_Be^{-itH_O} = \sum_{\nu\in\ZZ^{m_0}}e^{it\jap{\nu,\omega}}F_\nu.
$$
This shows that the limit defining $\HBbar$ exists, and is given by
$$
\HBbar = \sum_{\nu\in\ZZ^{m_0}:\jap{\nu,\omega}=0} F_\nu.
$$

As in the classical case, we may look for conditions under which the limiting motion can be considered
to take place on $\SS$. Suppose that the eigenvalues $\omega_1,\ldots,\omega_m$ are all distinct, and, in 
addition, that the eigenvectors $n_k(\ss)$ can be chosen to be smooth functions on all of $\SS$. Then
the normal bundle is trivial, $N\SS = \SS\times\RR^{m}$ and $L^2(N\SS, \dvns) = L^2(\SS,d{\rm vol}_\SS)\otimes L^2(\RR^m,d^my)$.
If the non-resonance condition \rf{nonres} holds, then
$$
\HBbar =  \left(-\half\L_\SS + V(\ss) + K(\ss)\right)\otimes 1 + V_1.
$$
The term $V_1$ is slightly different from \rf{V1}, because terms arising in its computation
do not all commute. It is given by 
$$
V_1 = \sum_{k,l}\left({{I_kI_l\omega_l}\over{\omega_k}} - {{1}\over{4}}\right)|b_{k,l}|^2.
$$
The joint eigenspaces of $I_1,\ldots, I_m$ are invariant subspaces for $\HBbar$. The restriction of 
$\HBbar$ to such a joint eigenspace is the Schr\"odinger operator $-\half\L_\SS + V(\ss) + K(\ss) + \tilde V_1$,
acting in $L^2(\SS,d{\rm vol}_\SS)$, where $\tilde V_1$ is obtained from $V_1$ by replacing the operators $I_k$
by their respective eigenvalues. Thus $\HBbar$ is a direct sum of Schr\"odinger operators acting in $L^2(\SS,d{\rm vol}_\SS)$.

\endsection


==> quantumpf2.tex <==
\beginproofof{\thmrf{quantum2}}
To prove the theorem, it suffices to show that for any $\psi\in C_0^\infty(N\SS)$,
$$
\lim_{\lambda\rarr\infty}\sup_{0\le t\le T}
\left\|\left(e^{-it(H_B+\lambda^2 H_O)} - e^{-it\lambda^2 H_O}e^{-it\HBbar}\right)\psi\right\|^2 = 0
$$
This can be rewritten as 
\be{goal}
\lim_{\lambda\rarr\infty}\sup_{0\le t\le T}
\left|\jap{\psi_{t,\lambda}-e^{-it\HBbar}\psi,e^{-it\HBbar}\psi}\right| = 0
\ee
where
$$
\psi_{t,\lambda} = e^{it\lambda^2 H_O}e^{-it(H_B+\lambda^2 H_O)}\psi
$$
We will show that for any $\varphi\in L^2(N\SS,\dvns)$
\be{goal2}
\sup_{0\le t\le T}\left|\jap{\psi_{t,\lambda}-e^{-it\HBbar}\psi,\varphi}\right| = 0,
\ee
which will imply \rf{goal}. 

This implication follows from the general fact that if $\psi_{t,\lambda}$ converges to some $\psi_{t,\infty}$ with 
$$
\sup_{0\le t\le T}\|\psi_{t,\infty}\| \le C
$$
in the sense that
$$
\sup_{0\le t\le T}\left|\jap{\psi_{t,\lambda}-\psi_{t,\infty},\varphi}\right| = 0
$$
then, for any continuous function $\varphi_t$ from $[0,T]$ into $L^2(N\SS,\dvns)$,
$$
\sup_{0\le t\le T}\left|\jap{\psi_{t,\lambda}-\psi_{t,\infty},\varphi_t}\right| = 0.
$$
To see this, pick
an orthonormal basis $\{\varphi_n\}$. Then
$$\displaylines{\quad
\sup_{0\le t\le T}\left|\jap{\psi_{t,\lambda}-\psi_{t,\infty},\varphi_t}\right|
\hfill\cr\hfill\eqalign{
&\le
\sup_{0\le t\le T}\left|\sum_{n=1}^N\jap{\psi_{t,\lambda}-\psi_{t,\infty},\varphi_n}
\jap{\varphi_n,\varphi_t}\right|
+\sup_{0\le t\le T}\left|\sum_{n=N+1}^\infty\jap{\psi_{t,\lambda}-\psi_{t,\infty},\varphi_n}
\jap{\varphi_n,\varphi_t}\right|\cr
&\le
C\sup_{0\le t\le T}\sum_{n=1}^N |\jap{\psi_{t,\lambda}-\psi_{t,\infty},\varphi_n}|
+C\sup_{0\le t\le T}\|(1-P_N)\varphi_t\|,
}\quad}$$
where $P_N$ denotes the orthogonal projection onto the span of $\varphi_1,\ldots,\varphi_N$. The first term on the right tends to zero as $\lambda\rarr\infty$, by assumption. Hence
$$
\limsup_{\lambda\rarr\infty}\sup_{0\le t\le T}\left|\jap{\psi_{t,\lambda}-\psi_{t,\infty},\varphi_t}\right|
\le C\sup_{0\le t\le T}\|(1-P_N)\varphi_t\|
$$
But $\{\phi_t: t \in [0,T]\}$ is compact and $1-P_N$
goes to zero uniformly on compact sets.
Therefore the right side tends to zero as $N\rarr\infty$. 

Thus it suffices to prove \rf{goal2}, which we will do in two steps. First, we will show that for every sequence $\lambda_j\rarr\infty$, there exists a subsequence $\mu_j$ and a bounded, weakly continuous $L^2(N\SS,\dvns)$ valued function $\psi_{t,\infty}$ such that
\be{step1}
\sup_{0\le t\le T}\left|\jap{\psi_{t,\mu_j}-\psi_{t,\infty},\varphi}\right|\rarr 0
\ee
for every $\varphi\in L^2(N\SS,\dvns)$. Then, to complete the proof, we will
show that $\psi_{t,\infty}$ is always the same, and equal to $e^{-it\HBbar}\psi$.

To take the first step, we begin with a sequence $\lambda_j\rarr\infty$.
Let $\{\varphi_n\}$ be an orthonormal basis of vectors in $C_0^\infty(N\SS)$. Define
$$
w_{n,\lambda}(t) = \jap{\psi_{t,\lambda},\varphi_n}
$$
Then for fixed $n$, $w_{n,\lambda}(t)$ are a family of functions of $t\in [0,T]$,
uniformly bounded as $\lambda\rarr\infty$. Still for fixed $n$, this family is equicontinuous,
since the derivative is bounded independently of $\lambda$. This follows from
$$\eqalign{
\left|{{d}\over{dt}} \jap{\psi_{t,\lambda},\varphi_n}\right| 
&= \left|-i\jap{e^{it\lambda^2 H_O}H_Be^{-it(H_B+\lambda^2 H_O)}\psi,\varphi_n}\right|\cr
&=\left|\jap{\psi_{t,\lambda},e^{it\lambda^2 H_O}H_Be^{-it\lambda^2 H_O}\varphi_n}\right|\cr
&\le \|\psi\|\cdot\|\sum_{\nu} e^{it\lambda^2\jap{\nu,\omega}}F_\nu \varphi_n\|\cr
&\le \|\psi\|\cdot \sum_{\nu} \|F_\nu \varphi_n\| = C_n\cr
}$$
The sum over $\nu$ is finite. Here we used \rf{HBexpansion}, and that $\varphi_n$ is in $C_0^\infty(N\SS)$, 
and therefore in the domain of $F_\nu$. 

Using Ascoli's theorem, we may now choose a subsequence $\lambda_{j_1}$
of $\lambda_j$ so that $w_{1,\lambda_{j_1}}(t)$ converges to some 
continuous function $w_{1,\infty}(t)$,
uniformly in $t$ for $t\in [0,T]$. Then we may choose a subsequence $\lambda_{j_2}$ of $\lambda_{j_1}$ with $w_{2,\lambda_{j_2}}(t)$ converging uniformly to some 
continuous function $w_{2,\infty}(t)$. Continuing in this way, and then taking a diagonal subsequence, we end up with 
a subsequence $\mu_j$ such that
$$
\sup_{0\le t\le T} \left|w_{n,\mu_j}(t) - w_{n,\infty}(t)\right| \rarr 0
$$
for every $n$. Notice that
$$\eqalign{
\sum_{n=1}^N|w_{n,\infty}(t)|^2 
&=\lim_{j\rarr\infty}\sum_{n=1}^N|\jap{\psi_{t,\mu_j},\varphi_n}|^2\cr
&\le \|\psi_{t,\mu_j}\|^2\cr
&= \|\psi\|^2\cr
}$$
This implies that $\sum_{n=1}^\infty|w_{n,\infty}(t)|^2 \le \|\psi\|^2$, so that
$$
\psi_{t,\infty} = \sum_n w_{n,\infty}(t)\varphi_n
$$
is well defined with $\|\psi_{t,\infty}\| \le \|\psi\|$. Clearly, for any $n$, $\jap{\psi_{t,\mu_j}-\psi_{t,\infty},\varphi_n}\rarr 0$ as
$j\rarr\infty$. This implies \rf{step1}

Now take the second step of identifying $\psi_{t,\infty}$. Let $\varphi\in C_0^\infty(N\SS)$. Then
\be{almostthere}\eqalign{
\jap{\psi_{t,\mu_j},\varphi} &= \jap{\psi,\varphi} 
+ i\int_0^t \jap{\psi_{s,\mu_j},e^{is\mu_j^2 H_O}H_Be^{-is\mu_j^2 H_O}\varphi}ds\cr
&= \jap{\psi,\varphi} 
+i\int_0^t \jap{\psi_{s,\infty},e^{is\mu_j^2 H_O}H_Be^{-is\mu_j^2 H_O}\varphi}ds\cr
&\hskip 100pt +i\int_0^t \jap{\psi_{s,\mu_j}-\psi_{s,\infty},e^{is\mu_j^2 H_O}H_Be^{-is\mu_j^2 H_O}\varphi}ds\cr
}\ee
Since $\varphi\in C_0^\infty(N\SS)$ the formula \rf{HBexpansion} implies that 
$$
|\jap{\psi_{s,\mu_j}-\psi_{s,\infty},e^{is\mu_j^2 H_O}H_Be^{-is\mu_j^2 H_O}\varphi}|
\le \sum_\nu |\jap{\psi_{s,\mu_j}-\psi_{s,\infty},F_\nu \varphi}|
$$
Thus the second term of \rf{almostthere} tends to zero as $j\rarr\infty$. On the other hand
$$\eqalign{
\lim_{j\rarr\infty} \int_0^t\jap{\psi_{s,\infty},e^{is\mu_j^2 H_O}H_Be^{-is\mu_j^2 H_O}\varphi}ds
&=\lim_{j\rarr\infty}\sum_\nu  \int_0^te^{is\mu_j^2\jap{\nu,\omega}}\jap{\psi_{s,\infty},F_\nu\varphi}ds\cr
&=\int_0^t\jap{\psi_{s,\infty},\HBbar\varphi}ds\cr
}$$
by the Riemann Lebesgue lemma. Thus, taking $j\rarr\infty$ in  \rf{almostthere} we obtain
\be{lastgasp}
\jap{\psi_{t,\infty},\varphi} = \jap{\psi,\varphi}+i\int_0^t\jap{\psi_{s,\infty},\HBbar \varphi}ds.
\ee
Now let $\tilde\varphi$ be in the domain of $\HBbar$.
Since $C_0^\infty$ is a core for $\HBbar$, we may use an approximation argument to replace $\varphi$ with
$e^{-is\HBbar}\tilde\varphi$ and $\HBbar \varphi$ with $\HBbar e^{-is\HBbar}\tilde\varphi$ in the equation above.
We find, using \rf{lastgasp},  
$$\eqalign{
{{d}\over{ds}}\jap{\psi_{s,\infty},e^{-is\HBbar}\tilde\varphi}
&={{d}\over{dt}}\jap{\psi_{t,\infty},e^{-is\HBbar}\tilde\varphi}\Big|_{t=s} + {{d}\over{dt}}\jap{\psi_{s,\infty},e^{-it\HBbar}\tilde\varphi}\Big|_{t=s}\cr
&=i\jap{\psi_{s,\infty},\HBbar e^{-is\HBbar}\tilde\varphi} - i\jap{\psi_{s,\infty},\HBbar e^{-is\HBbar}\tilde\varphi}\cr
&=0\cr
}$$
Thus $\jap{\psi_{s,\infty},e^{-is\HBbar}\tilde\varphi}$ is constant. But when $s=0$, equation \rf{lastgasp} implies $\jap{\psi_{s,\infty},e^{-is\HBbar}\tilde\varphi}=\jap{\psi,\tilde\varphi}$. Thus$\jap{e^{is\HBbar}\psi_{s,\infty}-\psi,\tilde\varphi}=0$
for every $\tilde\varphi$ in the domain of $\HBbar$. This implies $e^{is\HBbar}\psi_{s,\infty}=\psi$, or $\psi_{s,\infty}=e^{-is\HBbar}\psi$,
and completes the proof.
\endproofof


==> refs.tex <==
\beginsection
\shd{References}
\parindent = 0pt

[AD] L.~Andersson and B.K.~Driver, {\it Finite dimensional approximations to Wiener measure and path integral formulas on manifolds},  
J.~Funct.~Anal.~ {\bf 165}, no. 2 (1999) 430--498.

\par

[A1] V.I.~Arnold, {\it Mathematical Methods of Classical Mechanics,}
Springer-Verlag, 1978.
\par

[A2] V.I.~Arnold, V.V.~Kozlov and A.I.~Neishtadt, {\it Mathematical Aspects of Classical  and Celestial Mechanics,} Encyclop\ae dia of Mathematical sciences, Volume 3, Springer-Verlag, 1988.
\par

[BS] Bornemann and Sch\"utte, {\it Homogenization of Hamiltonian systems with a strong constraining potential,} Physica D, {\bf 102} (1997) 57-77
\par

[C] Paul R.~Chernoff, {\it Essential self-adjointness of powers of generators
of hyperbolic equations,} J. Functional Analysis vol.~12, (1973) 401-414 

[dC1] R.C.T.~da Costa, {\it Quantum mechanics of a constrained particle,}
Physical Review A, Volume 23 Number 4 (1981) 1982--1987.
\par

[dC2] R.C.T.~da Costa, {\it Constraints in quantum mechanics,}
Physical Review A, Volume 25 Number 6 (1982) 2893--2900.
\par

[D] E.B.~Davies, {\it The functional calculus,} J.~London Math.~Soc.~(2) {\bf 52} no.~1 (1995) 166--176.

[DE] P.~Duclos and P.~Exner, {\it Curvature-induced bound states in quantum waveguides in two and three dimensions,} Reviews in Mathematical Physics, {\bf 7}, no.~1 (1995) 73--102
\par

[FK] A.~Figotin and P.~Kuchment, {\it Spectral properties of classical waves in high contrast media,} SIAM Journal of Applied Mathematics, {\bf 58} (1998) 683--702
\par

[F] M.~Friedlin, {\it Markov Processes and Differential Equations: Asymptotic Problems,} Lectures in Mathematics ETH, Birkh\"auser, 1996.
\par

[FW] M.I.~Friedlin and A.D.~Wentzell, {\it Random Perturbations of Dynamical Systems,} second edition, Springer, 1998.

[FH] R.~Froese and I.~Herbst, {\it Realizing holonomic constraints in classical and quantum mechanics,} Proceedings of the 1999 VAB--GIT international conference on differential equations.
\par

[G] G.~Gallavotti, {\it The Elements of Mechanics,} Springer-Verlag, 1983.
\par

[GS] V.~Guillemin and S.~Sternberg, {\it Symplectic techniques in physics,}
Cambridge University Press, 1984.
\par

[HS1] B.~Helffer and J.~Sj\"ostrand, {\it Puits multiples en m\'echanique semi-classique V, \'Etude des mini-puits,} Current topics in partial differential equations, Kinokuniya Company Ltd., 133--186 (Volume in honour of S.~Mizohata)
\par

[HS2] B.~Helffer and J.~Sj\"ostrand, {\it Puits multiples en m\'echanique semi-classique VI, Cas des puits sous-vari\'et\'es,} Annales de l'Institut Henri Poincar\'e, Physique Th\'eorique, {\bf 46} no.~4 (1987) 353--372
\par

[KZ] P.~Kuchment and H.~Zeng, {\it Convergence of spectra of mesoscopic systems collapsing onto a graph,} preprint (mp\_arc preprint no.\ 00-308 at {\tt http://www.ma.utexas.edu/mp\_arc/})

[RU] H.~Rubin and P.~Ungar, {\it Motion under a strong constraining force,} Communications on pure and applied mathematics, {\bf 10} (1957) 28--42
\par

[S] M.~Schatzman, {\it On the eigenvalues of the Laplace operator on a thin set
with Neumann boundary conditions,} Applicable Analysis, {\bf 61} (1996) 293--306
\par


[Ta] F.~Takens, {\it Motion under the influence of a strong constraining force,}
in Global theory of dynamical systems, Springer lecture notes in mathematics,
{\bf 819} (1980) 425--445
\par

[To] J.~Tolar, {\it On a quantum mechanical d'Alembert principle,} Group theoretical methods in physics, Springer lecture notes in physics,
{\bf 313} (1988) 268--274
\par

\endsection


==> results.tex <==
\vfill\eject
\beginsection
\shd{Classical mechanics: bounded energy}

To give a precise statement of our results we must introduce some notation.
The normal bundle to $\SS$ is the submanifold of $\RR^{n+m}\times\RR^{n+m}$
given by
$$
N\SS =\{(\ss, n):\ss\in\SS,\,n\in N_\ss\SS\}
$$
Here $N_\ss\SS$ denotes the normal space to $\SS$ at $\ss$, identified with
a subspace of $\RR^{n+m}$. 

There is a natural map from $N\SS$ into
$\RR^{n+m}$ given by 
$$
\iota:(\ss,n)\mapsto \ss+n.
$$
We now fix a sufficiently small $\delta$ so that this map is a
diffeomorphism of $N\SS_\delta=\{(\ss,n):\|n\|<\delta\}$ onto a tubular
neighbourhood of $\SS$ in $\RR^{n+m}$. Then we can pull back the Euclidean
metric from $\RR^{n+m}$ to $N\SS_\delta$. Since we are interested in the
motion close to $\SS$ we may use $N\SS_\delta$ as the classical
configuration space. This will be convenient in what follows, and is justified below.

We will want to decompose vectors in the cotangent spaces of $N\SS_\delta$
into horizontal and vertical vectors, so we now explain this decomposition.
Let $\pi:N\SS\rarr \SS$ denote the projection of 
the normal bundle onto the base given by $\pi:(\ss, n)\mapsto \ss$.
The vertical subspace of $T_{\ss,n}N\SS$ is defined to be the kernel of
$d\pi: T_{\ss,n}N\SS\rarr T_\ss\SS$. The horizontal subspace is then defined 
to be the orthogonal complement (in the pulled back metric)
of the vertical subspace. Using the identification of $T_{\ss,n}N\SS$
with $T^*_{\ss,n}N\SS$ given by the metric we obtain a decomposition of cotangent vectors
into horizontal and vertical components as well. We will denote by $(\xi, \eta)$ the
horizontal and vertical components of a vector in $T^*_{(\ss,n)}N\SS$.

The decomposition can be explained more concretely as follows. 
For each point $\ss\in\SS$, we may decompose $T_\ss\RR^{n+m}=T_\ss\SS\oplus
N_\ss\SS$ into the tangent and normal space. Using the natural
identification of all tangent spaces with $\RR^{n+m}$, we may regard this as
a decomposition of $\RR^{n+m}$. Let $P_\ss^T$ and $P_\ss^N$ be the
corresponding orthogonal projections. Since we are thinking of $N\SS$ as an
$n+m$--dimensional submanifold of $\RR^{n+m}\times\RR^{n+m}$, we can
identify $T_{(\ss,n)}N\SS$  with the $n+m$--dimensional subspace of
$\RR^{n+m}\times\RR^{n+m}$ given by all vectors of the form
$(X,Y)=(\dot\ss(0),\dot n(0))$, where $(\ss(t),n(t))$ is a curve in $N\SS$
passing through $(\ss,n)$ at time $t=0$. The inner product of two such tangent
vectors is
\be{ip}
\jap{(X_1,Y_1),(X_2,Y_2)} = \jap{X_1+Y_1,X_2+Y_2}
\ee
where the inner product on the right is the usual Euclidean inner product.
For a tangent vector $(X,Y)$, the
decomposition into horizontal and vertical vectors is given by
$$
(X,Y) 
= (X,P_\ss^TY)+(0,P_\ss^NY)
$$

In the statements of our theorems we will want to express the fact that two
cotangent vectors, for example $\xi_\lambda(t)$ and $\xi(t)$ in \thmrf{classorig}, 
are close, even though they belong to two different cotangent 
spaces. To do this we may use the imbedding to think of the vectors as elements
of $\RR^{2(n+m)}$. Then it makes sense to use the (Euclidean) norm of their difference,
$\|\xi_\lambda(t)-\xi(t)\|$ to measure how close they are. We will use the symbol
$\|\cdot\|$ in this situation, while $|\xi|$ will denote the norm of $\xi$ as a cotangent
vector.



We will assume that the constraining potential is a $C^\infty$ function of the form
\be{quadform}
W(\ss,n) = \half \jap{n,A(\ss)n}
\ee
where for each $\ss$, $A(\ss)$ is a positive definite linear transformation on $N_\ss\SS$.
The Hamiltonian \rf{hamlambda} can then be written
\be{hamlambda2}
H_\lambda(\ss,n,\xi,\eta) = \half\jap{\xi,\xi} + \half\jap{\eta,\eta} + V(\ss+n) + {{\lambda^4}\over{2}}\jap{n, A(\ss)n}
\ee
Notice that on the boundary of $N\SS_{\delta_1}$, for $0<\delta_1<\delta$,
$$
H_\lambda(\ss,n,\xi,\eta) \ge c_1\lambda^4 - c_2
$$ 
with 
$$\eqalign{
c_1&=  \inf_{(\sigma,n):\sigma\in\SS, \|n\| = \delta_1} W(\sigma+n)>0\cr
c_2&= \sup _{(\sigma,n):\sigma\in\SS, \|n\| = \delta_1} |V(\ss+n)|\cr
}$$
By conservation of energy, this implies that an orbit under $H_\lambda$ that starts out in $N\SS_{\delta_1}$ with initial energy less than $c_1\lambda^4 - c_2$ can never cross the boundary, and therefore stays in $N\SS_{\delta_1}$. We will only consider such orbits in this paper, and therefore are justified in taking our phase space to be $T^*N\SS_\delta$, or even $T^*N\SS$ if we extend $H_\lambda$ in some arbitrary way.

Since we expect the motion in the normal directions to consist of rapid
harmonic oscillations, it is natural to introduce action variables for this
motion. There is one for each distinct eigenvalue $\omega_\alpha^2(\ss)$ of
$A(\ss)$.
Let $P_\alpha(\ss)$ be the projection onto
the eigenspace of $\omega_\alpha^2(\ss)$.  This projection is defined on
$N_\ss\SS$, which we may think of as the range of $P_\ss^N$ in $\RR^{n+m}$.
Thus the projection is defined on vertical vectors in $T_{(\ss,n)}N\SS$
and, via the natural identification, on vertical vectors in
$T^*_{(\ss,n)}N\SS$.  With this notation, the corresponding action variable,
multiplied by $\lambda^2$ for notational convenience,
is given by
\be{action}
I_\alpha^\lambda(\ss,n,\xi,\eta) = {{1}\over{2\omega_\alpha(\ss)}}\jap{\eta,P_\alpha \eta}
+{\lambda^4{\omega_\alpha(\ss)}\over{2}}\jap{n,P_\alpha n}
\ee
Notice that the total normal energy is given by $\sum_\alpha
\omega_\alpha I_\alpha^\lambda$.
The following is a version of the theorem of Takens and Rubin, Ungar.

\begintheoremlabel{classorig}
Let the Hamiltonian $H_\lambda$ be given by \rf{hamlambda2} where $V,W\in C^\infty$, $W$ has the form \rf{quadform} and satisfies
\par\indent (i) The eigenvalues $\omega_\alpha^2(\ss)$ of $A(\ss)$ have constant multiplicity.\par\noindent
Suppose that $(\ss_\lambda,n_\lambda,\xi_\lambda,\eta_\lambda)$ are initial conditions in $T^*N\SS_\delta$ satisfying
\par (a) $\| \ss_\lambda - \ss_{0}\| + \|\xi_\lambda - \xi_{0}\| \rarr 0$,
\par (b) $I_\alpha^\lambda(\ss_\lambda,n_\lambda,\xi_\lambda,\eta_\lambda) \rarr
I_\alpha^0 > 0$,
\par\noindent as  $\lambda\rarr\infty$. Let $(\ss_\lambda(t), n_\lambda(t),\xi_\lambda(t), \eta_\lambda(t))$ denote the subsequent 
orbit in $T^*N\SS_\delta$ under the Hamiltonian $H_\lambda$.

Suppose that $(\ss(t),\xi(t))$ is the orbit in $T^*\SS$ with initial conditions
$(\ss_{0},\xi_{0})$ governed by the Hamiltonian
$$
h(\ss,\xi) = \half\jap{\xi,\xi}_\ss + V(\ss) + \sum_\alpha I_\alpha^0\omega_\alpha(\ss).
$$

Then for any $T\ge 0$
$$
\sup_{0\le t\le T} \|\ss_\lambda(t)-\ss(t)\| 
+ \| \xi_\lambda(t)-\xi(t)\| \rarr 0
$$
as $\lambda\rarr\infty$. 
\endtheorem
Implicit in this statement is the fact that the approximating orbit stays
in the tubular neighbourhood for $0\le t\le T$, provided $\lambda$ is
sufficiently large. This theorem is actually true in greater generality. We
can consider smooth constraining potentials $W$ where $\half
\jap{n,A(\ss)n}$ is the first term in an expansion. If we choose our
tubular neighbourhood so that $W(\ss+n)\ge c |n|^2$ and impose the
non-resonance condition $\omega_\alpha(\ss) \ne
\omega_\beta(\ss)+\omega_\gamma(\ss)$ for every choice of $\alpha$, $\beta$
and $\gamma$ and for every $\ss$, then the same conclusion holds. This theorem
is also really a local theorem: if we impose the conditions on $W$ and the
non-resonance condition locally, and take $T$ to be a number less than the time where $\ss(t)$ 
leaves the set where condition {\it(i)} is true, then the same
conclusion holds as well.

Actually, Takens [T] only treats the case where all the eigenvalues $\omega_\alpha$
are distinct and the where the normal bundle is trivial. On the other hand,
he does not require that $I_\alpha^0 > 0$. This positivity is a technical requirement
of our proof and arises because action angle co-ordinates are singular on the 
surface $I_\alpha^0 = 0$. Since \thmrf{classorig} is a minor variation of known
results, we will not give a proof here.

\endsection

\beginsection
\shd{Classical mechanics: unbounded energy}

We now describe our theorems in classical mechanics where the initial
energies are diverging as they do in the quantum case. 
In quantum mechanics, the ground state energy of a harmonic oscillator
$-\half (d/dx)^2 + \half \lambda^4\omega^2 x^2$ is $\lambda^2\omega/2$. Thus
we will assume  that the initial values of the 
action variables $I_\alpha^\lambda$ scale like $\lambda^2I_\alpha^0$, 
and therefore that the initial normal energy
diverges like $\lambda^2$. Examining the effective 
Hamiltonian $h(\ss,\xi)$ in
\thmrf{classorig}, one
would expect there to be a diverging $\lambda^2\sum_\alpha
I_\alpha^0\omega_\alpha(\ss)$ potential term 
similar to the constraining potential but with strength $\lambda^2$.
If this potential is not constant, and thus has a local minimum 
(called a mini-well in [HS1, HS2]), 
no limiting orbit could be expected in general unless the
initial positions were chosen to converge to
such a minimum. 
For simplicity, we will assume that
there are no mini-wells, i.e., the frequencies $\omega_\alpha$ are constant.

The first step in our analysis is a large $\lambda$ expansion. It is
convenient to implement this expansion using dilations in the fibre of
the normal bundle. It is also convenient to assume that our configuration
space is all of $N\SS$. This makes no difference, since
the orbits we are
considering never leave $N\SS_\delta$. 

The dilation $d_\lambda:N\SS\rarr N\SS$ is defined by
$$
d_\lambda (\ss, n) = (\ss, \lambda n)
$$
As with any diffeomorphism of the configuration space, $d_\lambda$ has a symplectic lift 
$D_\lambda$ to the cotangent bundle given by
$$
D_\lambda = d_{\lambda}^{-1 *} = d_{\lambda^{-1}}^{*}
$$
The expression for $D_\lambda$ in local co-ordinates is given by \rf{Dlc}.


Instead of the original Hamiltonian $H_\lambda$ we may now consider
the equivalent pulled back Hamiltonian $L_\lambda=H_\lambda\circ D_\lambda^{-1}$.
Since $D_\lambda$ is a symplectic transformation, orbits under $H_\lambda$ and orbits under $L_\lambda$
are mapped to each other by $D_\lambda$ and its inverse. Therefore,
it suffices to study the dynamics of the scaled Hamiltonian $L_\lambda$.

A formal large $\lambda$ expansion yields
$$
L_\lambda
= H_B + \lambda^2 H_O + O(\lambda^{-1})
$$
where $H_O$ is the harmonic oscillator Hamiltonian
\be{HOorig}
H_O(\ss,n,\xi,\eta)= \half\jap{\eta,\eta} + \half\jap{n,A(\ss) n}
\ee
and $H_B$ is the bundle Hamiltonian given by
\be{HBorig}
H_B(\ss,n,\xi,\eta)=\half\jap{J\xi,J\xi}_\ss
+V(\ss)
\ee
The inner product $\jap{\cdot,\cdot}_\ss$ is the inner product on $T^*\SS$
defined by the imbedding. 
Here $J$ denotes the identification of the horizontal subspace of $T^*_{\ss,n}N\SS$
with the horizontal subspace of $T^*_\ss\SS$ given in terms of the bundle projection map
$\pi_{\ss,n}$ by $J=d\pi_{\ss,n}^{* -1}.$ This map is well defined on the horizontal subspace,
since  $d\pi_{\ss,n}: T_{\ss,n}N\SS\rarr T_\ss\SS$
is an isomorphism when restricted to the 
horizontal subspace of $T_{\ss,n}N\SS$. Thus, its adjoint $d\pi_{\ss,n}^*$ is 
an isomorphism of $T^*_\ss\SS$ onto the horizontal subspace of $T^*_{\ss,n}N\SS$.
In local co-ordinates $x_i, y_i$ defined in section 5 below, where $x_i$ are co-ordinates for $\SS$,
the map $J$ simply identifies $dx_i\in T^*_{\ss,n}N\SS$ with $dx_i\in T^*_\ss\SS$.

Additional understanding of the Hamiltonians $H_B$  and $H_O$can be obtained if we introduce another metric on 
$N\SS$. 
If $(X,Y)\in T_{(\ss,n)}N\SS$,
let
\be{newmetric}
\jap{(X,Y),(X,Y)}_\lambda = \|X\|^2 + \lambda^{-2}\|P_\ss^NY\|^2.
\ee
(In Section 7 we describe in what sense this is a limiting form of the pulled-back, scaled, Euclidean metric.) 
If $\jap{\cdot,\cdot}^\lambda$ denotes the corresponding metric on the cotangent space, then
$$
H_B + \lambda^2H_O = \half\jap{(\xi,\eta),(\xi,\eta)}^\lambda + {{\lambda^2}\over{2}}\jap{n,A(\ss)n} + V(\ss)
$$
The local co-ordinate expressions for $H_B$ and $H_O$ are 
given in \rf{HB} and \rf{HO}.



%Here $f\in T^*_\ss\SS$ is defined locally as follows. Choose a local
%co-ordinate system $x\mapsto \ss(x)$ for $\SS$ and local
%frame $n_1(\ss),\ldots,n_m(\ss)$ for the normal bundle. Then we obtain
%local co-ordinates for $N\SS$ by sending $(x,y)\mapsto (\ss(x),\sum
%y_kn_k)$. (Here $n_k$ denotes $n_k(\ss(x))$.) 
%Associated with the frame is the connection one-form. This is the antisymmetric matrix valued one-form given by
%\be{connform}
%b_{k,l}[\cdot]=\jap{n_k,dn_l[\cdot]}
%\ee 
%(Here we are thinking of $n_k$ as a map
%from $\SS$ to $\RR^{n+m}$, and the inner product is in $R^{n+m}$.)
%With this notation,
%$$
%f(\ss(x),\sum y_kn_k,\sum r_k dy_k)[\cdot]=
%\sum_{k,l} y_kb_{k,l}[\cdot]r_l.
%$$

%The following theorem describes a sequence of orbits with initial conditions $\gamma_\lambda\in T^*N\SS$ %obeying 
%$$D_\lambda\gamma_\lambda\rarr\gamma_0.$$
%If $\gamma_\lambda = (\ss_\lambda,n_\lambda,\xi_\lambda,\eta_\lambda)$, this condition implies that
%\par 
%(a) $\ss_\lambda \rarr \ss_0$, \par 
%(b) $\lambda n_\lambda \rarr  n_0$, \par
%(c) $\xi_\lambda \rarr d\pi^{* -1}\xi_0 + f(\sigma_0, n_0, \eta_0)$, \par 
%(d) $\lambda^{-1}\eta_\lambda \rarr \eta_0$.\par\noindent
%(Here we are thinking of $\ss$, $n$ as vectors in $\RR^{n+m}$ and
%$\xi$, $\eta$ as vectors in $\RR^{2(n+m)}$.) 
%So, although the initial position is converging to a point on $\SS$, the initial
%normal energy $\sum I_\alpha^\lambda$ is diverging like $\lambda^2$.

We will use the notation $\phi^H_t$ to denote the Hamiltonian flow governed by
the Hamiltonian $H$.

\begintheoremlabel{classical1}
Let $L_\lambda=H_\lambda\circ D_\lambda^{-1}$, where the Hamiltonian $H_\lambda$ is given by \rf{hamlambda2}.
Assume that
$V,W\in C^\infty$,  $W$ has the
form \rf{quadform}, and  that the eigenvalues $\omega_\alpha^2$ of $A(\ss)$ do not
depend on $\ss$.\par\noindent
Suppose that $\gamma_{\lambda}$ are initial
conditions in $T^*N\SS$ with
$\gamma_{\lambda}\rarr\gamma_0$
as  $\lambda\rarr\infty$. 

Then for any $T\ge 0$
$$
\sup_{0\le t\le T} \left\|\phi^{L_\lambda}_t(\gamma_\lambda)-\phi^{H_B+\lambda^2 H_0}_t(\gamma_0)\right\| \rarr 0
$$
as $\lambda\rarr\infty$. 
\endtheorem
 
In this theorem the normal energy of the initial conditions,
$\lambda^2H_O(\gamma_{\lambda})$ grows like $\lambda^2$,
since $H_O(\gamma_{\lambda})$ is converging to $H_O(\gamma_0)$. 
This leads to increasingly rapid normal oscillations for both orbits 
$\phi^{L_\lambda}_t(\gamma_\lambda)$ and $\phi^{H_B+\lambda^2 H_0}_t(\gamma_0)$.
Neither orbit  converges as $\lambda$
becomes large. It is only their difference that converges.

The convergence of the initial conditions is stated for the scaled
variables $\gamma_\lambda$. To find out what this implies for the original variables
$(\tilde \ss_\lambda, \tilde n_\lambda, \tilde \xi_\lambda, \tilde \eta_\lambda) = D_\lambda^{-1}\gamma_\lambda$ we must determine the 
action of $D_\lambda$ on horizontal and vertical vectors. This results in
the following conditions
\par 
(a) $\tilde \ss_\lambda \rarr \ss_0$, \par 
(b) $\lambda \tilde n_\lambda \rarr  n_0$, \par
(c) $\tilde \xi_\lambda \rarr J\xi_0$, and \par 
(d) $\lambda^{-1}\tilde \eta_\lambda \rarr \eta_0$\par\noindent
where $(\ss_0,n_0,\xi_0,\eta_0)=\gamma_0$. Here we are thinking of $\ss$, $n$ as vectors in $\RR^{n+m}$ and
$\xi$, $\eta$ as vectors in $\RR^{2(n+m)}$. We may also compute what these conditions mean for the initial
velocities $(X_\lambda,Y_\lambda)\in T_{\tilde\ss_\lambda, \tilde n_\lambda}N\SS$, again thought of as vectors in $\RR^{2(n+m)}$.
It turns out that\par
(c') $X_\lambda\rarr X_0$, and\par 
(d') $\lambda^{-1}Y_\lambda\rarr Y_0$.


This theorem gives a satisfactory description of the limiting motion if the
Poisson bracket of $H_B$ and $H_O$ vanishes. 
Then the flows generated by $H_B$
and $H_O$ commute and the motion is given by the rapid oscillations
generated by $\lambda^2H_O$ superimposed on the flow generated by $H_B$.
In this
situation we can perform averaging by simply ignoring the oscillations.

An example where $\{H_B,H_O\}$ is zero 
is when $\SS$ has codimension one, or, more generally, if the
connection form vanishes. Then $H_B $ only
involves variables on $T^*\SS$, so the motion for large $\lambda$ is a motion on
$\SS$ with independent oscillations in the normal variables. 
The Poisson bracket $\{H_B,H_O\}$ also vanishes if all the frequencies
$\omega_\alpha$ are equal, but in this case the motion generated by $H_B$ need
not only involve the variables on $T^*\SS$.

The motion generated by $H_B$ can be
thought of as a generalized minimal coupling type flow. (See [GS] for a
description of the geometry of this sort of flow.) The flow has the
property that the trajectories in $N\SS$ are parallel along their
projections onto $\SS$. In particular, $|n|^2$ is preserved by this motion.


In general, when the frequencies are not all equal, the flows generated by
$H_B$ and $\lambda^2H_O$ interact, and $H_B+\lambda^2H_O$ generates a more complicated
flow which need not be simply related to the flows generated by $H_B$ and $H_O$.
Let $\HBbar$ defined by
\be{HBbar}
\HBbar(\gamma) = \lim_{T\rarr\infty}T^{-1}\int_0^T H_B\circ\phi_t^{H_O}(\gamma) dt.
\ee
The existence of this limit follows from the Fourier expansion discussed
below.
This averaged Hamiltonian Poisson commutes with $H_O$. It turns out that the 
flow for large $\lambda$ is the one generated by this Hamiltonian, with superimposed normal oscillations.

\begintheoremlabel{classical2}
Assume that the assumptions of \thmrf{classical1} hold.
Let $H_O$, $H_B$ and $\HBbar$ be the Hamiltonians given by \rf{HOorig}, \rf{HBorig} and 
\rf{HBbar} respectively. Let $\gamma_0\in T^*{N\SS}$ and $T>0$. Then
\be{cl2est}
\sup_{0\le t\le T} \left\|\phi^{H_B+\lambda^2 H_0}_t(\gamma_0) 
			- \phi^{\lambda^2 H_0}_t\circ\phi^{\HBbar}_t(\gamma_0)\right\| \rarr 0
\ee
as $\lambda\rarr\infty$. 
\endtheorem

In this theorem we do not impose a non-resonance condition. However, 
the form of the averaged Hamiltonian $\HBbar$ depends crucially on whether or not resonances are present.

To explain this further we introduce scaled action variables. Recall that the scaled
Hamiltonian was defined by $L_\lambda=H_\lambda\circ D_\lambda^{-1}$. We perform
a similar scaling on the action variables and define $I_\alpha$ by
$$
I_\alpha^\lambda\circ D_\lambda^{-1} = \lambda^2 I_\alpha.
$$
Then
$$
I_\alpha(\ss,n,\xi,\eta) = {{1}\over{2\omega_\alpha}}\jap{\eta,P_\alpha \eta}
+{{\omega_\alpha}\over{2}}\jap{n,P_\alpha n}.
$$

Suppose that there are $m_0$ distinct eigenvalues $\omega^2_\alpha$.
Then the flows $\phi_t^{I_\alpha}$ are commuting harmonic oscillations in
the normal variables. They are periodic, satisfying $\phi_{t+2\pi}^{I_\alpha}=\phi_t^{I_\alpha}$
We therefore obtain a group action $\Phi$ of the $m_0$ torus $T^{m_0}$ on $T^*N\SS$ defined by
$$
\Phi_\tau= \phi_{\tau_1}^{I_1}\circ\cdots\circ\phi_{\tau_{m_0}}^{I_{m_0}},
$$
for $\tau = (\tau_1,\ldots,\tau_{m_0})\in T^{m_0}$. Notice that $\phi^{H_O}_t = \Phi_{t\omega}$ where
$\omega=(\omega_1,\ldots,\omega_{m_0})$.

Now we may perform a Fourier expansion of $H_B\circ\Phi_\tau$ yielding
$$
H_B\circ\Phi_\tau = \sum_{\nu\in\ZZ^{m_0}} e^{i\jap{\nu,\tau}} F_\nu
$$
so that
$$
H_B\circ\phi^{H_O}_t = \sum_{\nu\in\ZZ^{m_0}} e^{it\jap{\nu,\omega}} F_\nu
$$
It turns out that only finitely many $F_\nu$'s are non-zero. Thus we may
exchange the integral and limit in the definition of $\HBbar$ with the Fourier sum
to obtain
$$
\HBbar = \sum_{\nu\in\ZZ^{m_0}} \left(\lim_{T\rarr\infty}T^{-1}\int_0^Te^{it\jap{\nu,\omega}}dt\right)F_\nu
= \sum_{\nu\in\ZZ^{m_0}:\jap{\nu,\omega}=0} F_\nu.
$$
The non-resonance condition on the eigenvalues $\omega = (\omega_1,\ldots,\omega_{m_0})$ in this situation would be
\be{origNR} 
\hbox{If $\nu \ne 0$ and $F_\nu \ne 0$ then $\jap{\nu,\omega} \ne 0$.}
\ee
If this condition holds, we find that $\HBbar=F_0$. 


We now examine the case $m_0=m$, where there are $m$ distinct frequencies $\omega_\alpha$.
We wish to describe how the limiting motion generated by $\HBbar$ can be thought of as taking place on $\SS$.
To begin, since $\{\HBbar,I_\alpha\}=0$ for each $\alpha$, each $I_\alpha$ is a constant of the motion, 
so the motion takes place on the level sets of $I_1,\ldots,I_m$. Furthermore, we want to
to disregard the normal oscillations. Technically, we may do this by replacing the original  phase
space $T^*N\SS$, with its quotient by the group action $\Phi$. This amounts to 
ignoring the angle variables in local action angle co-ordinates. 

It turns out that
\be{psid}
T^*N\SS / \Phi = T^*\SS \times \RR^{m},
\ee
where the
variables in $\RR^{m}$ are the action variables. Since these are constant, we may think
of the motion as taking place on $T^*\SS$. To describe the identification \rf{psid} we 
first make a new direct sum decomposition of each cotangent space $T^*_{(\ss,n)}N\SS$. Since there are $m$ 
distinct eigenvalues $\omega_1,\ldots,\omega_m$, the corresponding eigenvectors, defined globally up to sign, give
an orthonormal frame for the normal bundle. In this situation the co-ordinates $y_i = \jap{n,n_i(\ss)}$ are also globally defined
up to sign. Thus the subspace of $T^*_{(\ss,n)}N\SS$ spanned by $dy_1,\ldots, dy_m$ is
globally defined. This subspace is complementary to the horizontal subspace, but is not 
necessarily  orthogonal. Given horizontal and vertical components $(\xi, \eta)$ of
a vector in $T^*_{(\ss,n)}N\SS$, we may write $\xi+\eta=\xi_1+\eta_1$ where $\xi_1$ is 
horizontal and $\eta_1$ is in the span of $dy_1,\ldots, dy_m$. 
The map from $T^*N\SS\rarr T^*\SS \times \RR^{m}$  given by
$$
(\ss,n,\xi,\eta)\mapsto(\ss,J\xi_1,I_1(\ss,n,\xi,\eta),\ldots,I_m(\ss,n,\xi,\eta))
$$
is invariant under $\Phi$ and gives rise to the identification \rf{psid}. 

Now suppose that the values of $I_1,\ldots, I_m$ have been fixed by the initial condition.
Then the Hamiltonian governing the motion on $T^*\SS$ depends on these ``hidden'' variables,
and is given by
\be{hB}
h_B(\ss,\xi;I_1,\ldots,I_m) = \half \jap{\xi,\xi}_\ss + V(\ss) + V_1(\ss;I_1,\ldots,I_m),
\ee
provided the  non-resonance condition holds. Given that the eigenvalues are distinct, the following implies \rf{origNR}
\be{nonres}\eqalign{
&\hbox{If $j\ne k$ and $l\ne m$ then $\omega_j \pm \omega_k \pm\omega_l\pm\omega_m\ne 0$}\cr
}\ee
The extra potential $V_1$ is defined in terms of the 
frame for the normal bundle, $n_1(\ss),\ldots, n_m(\ss)$, consisting of normalized eigenvectors of $A(\ss)$. 
Let $b_{k,l}$ be the associated connection one-form given by 
\be{connform}
b_{k,l}[\cdot]=\jap{n_k,dn_l[\cdot]}
\ee
Then
\be{V1}
V_1(\ss;I_1,\ldots,I_m)=\sum_{k,l}{{I_kI_l\omega_l}\over{\omega_k}}|b_{k,l}|^2.
\ee
Notice that the norm $|b_{k,l}|$ is insensitive to the choice of signs for
the frame.


\endsection


==> rixmax.tex <==
\input amssym.def
%\def\Bbb{\bf} %if \Bbb not available
 
%fonts

\font\bold=cmssbx10
\font\smallfont = pplr at 8.5pt
\font\smallit = pplri at 8.5pt
\font\normalfont = pplr at 9.5pt
\font\it = pplri at 9.5pt
\font\marginfont=cmr7


% shorthand
 
\def\larr{\leftarrow}
\def\rarr{\rightarrow}
\def\uarr{\uparrow}
\def\darr{\downarrow}
\def\PA{\partial}
\def\ti{\tilde}
\def\<{\langle}
\def\>{\rangle}
\def\cents{\hbox{\rm\rlap/c}}

% single letters

\def\HI{{\cal H}}
\def\HH{{\Bbb H}}
\def\RR{{\Bbb R}}
\def\CC{{\Bbb C}}
\def\ZZ{{\Bbb Z}}
\def\NN{{\Bbb N}}
\def\MM{{\cal M}}
\def\QQ{{\Bbb Q}}
\def\DD{{\cal D}}
\def\FF{{\cal F}}
\def\BB{{\cal B}}
\def\GG{{\cal G}}
\def\SS{{\bf S}}
\def\TT{{\bf T}}
\def\EE{{\cal E}}
\def\UU{{\cal U}}
\def\II{{\cal I}}
\def\OO{{\cal O}}

% misc math stuff

\def\slim{\mathop{\hbox{\rm s-lim}}}
\def\Ker{\mathop{\rm Ker}}
\def\Ran{\mathop{\rm Ran}}
\def\ad{\mathop{\rm ad}}
\def\Re{\mathop{\rm Re}}
\def\Im{\mathop{\rm Im}}
\def\ess{\hbox{\it ess}}
\def\d{\hbox{\it d}}
\def\c{\hbox{\it c}}
\def\pp{\hbox{\it pp}}
\def\jap#1{\langle #1 \rangle}
\def\sph{S^{n\kern -.2ex -\kern -.2ex 1}}
\def\half{$\scriptstyle{{1}\over{2}}$}
\def\DT{{{\partial}\over{\partial t}}}
\def\L{\Delta}
\def\norm#1{\|#1\|}
\def\amat4#1#2#3#4#5#6#7#8{
\left[\matrix{
#1\cr
#3\cr
#5\cr
#7\cr
}\right.\left|\matrix{
#2\cr#4\cr#6\cr#8\cr
}\right]
}
\def\vec4#1#2#3#4{
\left[\matrix{
#1\cr
#2\cr
#3\cr
#4\cr
}\right]
}

\def\amat3#1#2#3#4#5#6{
\left[\matrix{
#1\cr
#3\cr
#5\cr
}\right.\left|\matrix{
#2\cr#4\cr#6\cr
}\right]
}
\def\vec3#1#2#3{
\left[\matrix{
#1\cr
#2\cr
#3\cr
}\right]
}
 
% misc


%
% 	the stuff after \ifdraftmode only appears if \draftmode has previously 
%	appeared
%
\def\draftmode{\let\dfmd 1}
\def\ifdraftmode#1{\ifx\dfmd 1{#1}\fi}

\def\today{\ifcase\month\or January\or February \or March \or April\or May\or June\or July\or August\or September\or October \or November \or December\fi
\space\number\day, \number\year}

\def\nnarrower{\advance\leftskip by 30pt\advance\rightskip by 30pt}

\def\wwider{\advance\leftskip by -30pt\advance\rightskip by -30pt}

\def\quote#1{{\smallskip\nnarrower\noindent{\it#1}\smallskip}}

\def\hd#1{\bigskip\bigskip{\noindent\bold #1}\par\vrule height\bigskipamount width 0pt\penalty10000}

\def\enum#1{\par\noindent\quad\rlap{#1}\hskip 20pt}

\def\Box{\vbox{\hrule
              \hbox{\vrule height7pt\kern7pt\vrule height7pt}
              \hrule
              }
        }

\def\Picbox{\centerline{
		\vbox{\hrule
                \hbox{\vrule height2.5in\kern5in\vrule height2.5in}
                \hrule
                }
	    }
        }

% 
%	a box of specified height, width and thickness
%

\def\boxhwt#1#2#3{\vbox{\hrule width#2 height#3
                	\hbox{\vrule height#1 width#3 \kern#2\kern-#3\kern-#3 \vrule height#1 width#3}
                	\hrule width#2 height#3
                	      }
        	}
%
%
%	mcomment puts a comment in the margins
%
%
%
%
\def\strutdepth{\dp\strutbox}
%
\newdimen\pagewidth
\newdimen\marginsize

\def\margininsert#1{\strut\vadjust{\kern-\strutdepth
\vtop to \strutdepth{\baselineskip\strutdepth\vss\llap{\marginfont #1}\null}}}
%
\def\marginbox#1{{
\pagewidth=8.5 true in
%	set \marginsize to 1in + \hoffset - .26 true in
	\marginsize=1 true in
	\advance \marginsize by \hoffset
	\advance \marginsize by -.26 true in
\parindent=0pt\raggedright\hsize = \marginsize\vbox{#1}\kern 3pt}}
%
%
\def\mcomment#1{\margininsert{\marginbox{#1}}}

%
%       the following macros read in the files \jobname.eqr 
%       and \jobname .thm which 
%       contain the names of equations and how they are nested 
%       within sections in a format like 
%       \\{name1}\bgnscn\\{name2}\bgnscn\\{name3}\ndscn\ndscn
%       In this example \eqlabelname1 will expand to 1
%                       \eqlabelname2 will expand to 1.1
%                       \eqlabelname3 will expand to 1.1.1
%       This is the maximum nesting supported
%       In the theorem list each \\{name} is preceded by \typetheorem,
%       \typelemma or \typeproposition to indicate what it is
%



\def\bgnsctn{
        \advance\secnest by1
        \cntnumber=0
        \ifnum\secnest=1 
                \advance\seclevelone by1 
                \edef\prenum{\number\seclevelone .}
        \fi
        \ifnum\secnest=2 
                \advance\secleveltwo by1
                \edef\prenum{\number\seclevelone .\number\secleveltwo .}
        \fi
        }
\def\ndsctn{\advance\secnest by-1}

\def\thmtype{} %initialize
\def\typetheorem{\def\thmtype{Theorem}}
\def\typelemma{\def\thmtype{Lemma}}
\def\typeproposition{\def\thmtype{Proposition}}
\def\typecorollary{\def\thmtype{Corollary}}
\def\typehypothesis{\def\thmtype{Hypothesis}}
\def\typeconjecture{\def\thmtype{Conjecture}}
%
% first do the references - define \\ to be a macro which defines \eqlabelname 
% to be a reference number and then evaluate the input string as in Appendix D
%
\def\\#1{
        \advance\cntnumber by1
        \expandafter\xdef\csname 
        eqlabel#1\endcsname{\prenum\number\cntnumber}
        }
\newcount\seclevelone \seclevelone=0
\newcount\secleveltwo \secleveltwo=0
\newcount\cntnumber \cntnumber=0
\newcount\secnest \secnest=0
\def\prenum{}
\newread\eqrinfile 
\openin\eqrinfile=\jobname .eqr 
\ifeof\eqrinfile
  \def\eqrinput{\relax}
\else\loop
  \read\eqrinfile to\eqrinput
  \eqrinput
  \ifeof\eqrinfile\let\endfile 1\else\let\endfile 0\fi
  \ifx\endfile 0 \repeat
\fi
\closein\eqrinfile

%
% now the same thing for theorems
%
\def\\#1{
        \advance\cntnumber by1
        \expandafter\xdef\csname 
        thmlabel#1\endcsname{\prenum\number\cntnumber}
        \expandafter\xdef\csname 
        typethmlabel#1\endcsname{\thmtype\ \prenum\number\cntnumber}
        }
\seclevelone=0
\secleveltwo=0
\cntnumber=0
\secnest=0
\def\prenum{}
\newread\thminfile 
\openin\thminfile=\jobname .thm
\ifeof\thminfile
  \def\thminput{\relax}
\else\loop
  \read\thminfile to\thminput
  \thminput
  \ifeof\thminfile\let\endfile 1\else\let\endfile 0\fi
  \ifx\endfile 0 \repeat
\fi
\closein\thminfile


        
%
% theorems etc
% These are numbered by section
%

\def\begintheoremlabel#1{
       	\toksdef\ta=0
	\ta={\typetheorem\\{#1}}
        \immediate\write\thmoutfile{\the\ta}
        \medbreak\par\noindent{\ifdraftmode{\mcomment{#1}}\bf Theorem \csname thmlabel#1\endcsname}
        \begingroup \it
}
\def\endtheoremlabel{\par\medbreak\endgroup}

\def\begintheorem{
        \advance\nonamectr by1
        \edef\temp{{noname\the\nonamectr}}
        \expandafter\begintheoremlabel\temp
}
\def\endtheorem{\endtheoremlabel}

\def\beginlemmalabel#1{
        \toksdef\ta=0
	\ta={\typelemma\\{#1}}
        \immediate\write\thmoutfile{\the\ta}
        \medbreak\par\noindent{\ifdraftmode{\mcomment{#1}}\bf Lemma \csname thmlabel#1\endcsname}
        \begingroup \it
}
\def\endlemmalabel{\par\medbreak\endgroup}

\def\beginlemma{
        \advance\nonamectr by1
        \edef\temp{{noname\the\nonamectr}}
        \expandafter\beginlemmalabel\temp
}
\def\endlemma{\endlemmalabel}



\def\beginpropositionlabel#1{
        \toksdef\ta=0
	\ta={\typeproposition\\{#1}}
        \immediate\write\thmoutfile{\the\ta}
        \medbreak\par\noindent{\ifdraftmode{\mcomment{#1}}\bf Proposition \csname thmlabel#1\endcsname}
        \begingroup \it
}
\def\endpropositionlabel{\par\medbreak\endgroup}

\def\beginproposition{
        \advance\nonamectr by1
        \edef\temp{{noname\the\nonamectr}}
        \expandafter\beginpropositionlabel\temp
}
\def\endproposition{\endpropositionlabel}

\def\begincorollarylabel#1{
        \toksdef\ta=0
	\ta={\typecorollary\\{#1}}
        \immediate\write\thmoutfile{\the\ta}
        \medbreak\par\noindent{\ifdraftmode{\mcomment{#1}}\bf Corollary \csname thmlabel#1\endcsname}
        \begingroup \it
}
\def\endcorollarylabel{\par\medbreak\endgroup}

\def\begincorollary{
        \advance\nonamectr by1
        \edef\temp{{noname\the\nonamectr}}
        \expandafter\begincorollarylabel\temp
}
\def\endcorollary{\endcorollarylabel}

\def\beginhypothesislabel#1{
        \toksdef\ta=0
	\ta={\typehypothesis\\{#1}}
        \immediate\write\thmoutfile{\the\ta}
        \medbreak\par\noindent{\ifdraftmode{\mcomment{#1}}\bf Hypothesis \csname thmlabel#1\endcsname}
        \begingroup \it
}
\def\endhypothesislabel{\par\medbreak\endgroup}

\def\beginhypothesis{
        \advance\nonamectr by1
        \edef\temp{{noname\the\nonamectr}}
        \expandafter\beginhypothesislabel\temp
}
\def\endhypothesis{\endhypothesislabel}

\def\beginconjecturelabel#1{
       	\toksdef\ta=0
	\ta={\typeconjecture\\{#1}}
        \immediate\write\thmoutfile{\the\ta}
        \medbreak\par\noindent{\ifdraftmode{\mcomment{#1}}\bf Conjecture \csname thmlabel#1\endcsname}
        \begingroup \it
}
\def\endconjecturelabel{\par\medbreak\endgroup}

\def\beginconjecture{
        \advance\nonamectr by1
        \edef\temp{{noname\the\nonamectr}}
        \expandafter\beginconjecturelabel\temp
}
\def\endconjecture{\endconjecturelabel}





\def\beginproof{\medbreak\par\noindent{\it Proof:\/\ }}
\def\endproof{\thinspace\Box\par\medbreak}

\def\beginproofof#1{\medbreak\par\noindent{\it Proof of #1:\/\ }}
\def\endproofof{\thinspace\Box\par\medbreak}



\def\begindefn{\medbreak\par\noindent{\it Definition:\/\ }}
\def\enddefn{\par\medbreak}

%\def\beginexample{\medbreak\par\noindent{\it Example:\/\ }}
%\def\endexample{\par\medbreak}

\def\beginexample{\beginproblemset\medbreak\par\noindent{\it Example:\/\ }}
\def\endexample{\par\medbreak\endproblemset}

\def\beginremark{\medbreak\par\noindent{\it Remark:\/\ }}
\def\endremark{\par\medbreak}



%-------------------------------------------------------
%	no longer needed
%
%       \appendtxt appends the text in #2 to the token list 
%       contained in the token variable #1
%
\def\appendtxt#1#2{ 
        \toksdef\ta=0
        \ta=\expandafter{\the#1#2}
        \global#1=\expandafter{\the\ta}
        }
%----------------------------------------------------------

%
%
%	open files for writing
%
%
\newwrite\eqroutfile 
\immediate\openout\eqroutfile=\jobname .eqr 
\newwrite\thmoutfile 
\immediate\openout\thmoutfile=\jobname .thm


%
%       \be{name} and \ee begin and end a numbered displayed equation 
%       the tokens in the name are added to the token list in \eqrtoks
%       if \eqlabelname has been defined uses this as a number
%       \lastdisplayline{name}{...} gives a referenced number  to the last 
%       line in a displaylines series
%
\def\be#1{
        \def\temp{#1}
	\toksdef\ta=0
	\ta={\\{#1}}
        \immediate\write\eqroutfile{\the\ta}$$
	}
\def\ee{
        \eqno{(\csname eqlabel\temp\endcsname)
	\ifdraftmode{\rlap{\ {\marginfont\temp}}}}$$
        }
\def\lastdisplayline#1#2{
        \hfill#2\hfill{\rm\llap{(\csname eqlabel#1\endcsname)}
	\ifdraftmode{\rlap{\ {\marginfont#1}}}}\cr
        \toksdef\ta=0
	\ta={\\{#1}}
        \immediate\write\eqroutfile{\the\ta}
        }

%
%       \beginsection begins a new section
%       writes \bgnsctn to token list in \eqrtoks
%       \endsection ends a section
%       writes \ndsctn to token list in \eqrtoks
%
\def\beginsection{
        \advance\secnumber by1
        \probctr=0
	\toksdef\ta=0
	\ta={\bgnsctn}
        \immediate\write\eqroutfile{\the\ta}
        \immediate\write\thmoutfile{\the\ta}
        }
\def\endsection{
        \toksdef\ta=0
	\ta={\ndsctn}
        \immediate\write\eqroutfile{\the\ta}
        \immediate\write\thmoutfile{\the\ta}
        }

%
%       \rf{name} inserts (<number>) where <number> is the equation number
%       referred to by "name"
%
\def\rf#1{(\csname eqlabel#1\endcsname )}

%
%       \thmrf is the analogous thing for theorems
%
\def\thmrf#1{\hbox{\csname typethmlabel#1\endcsname}}







\def\chead#1{\medbreak\centerline{#1}\medskip}

\def\bea#1{$$\eqalign\begingroup}
\def\eea{\endgroup $$}
\def\beann{$$\eqalign\begingroup}
\def\eeann{\endgroup $$}


%
%       some lecture note macros
%
\def\beginlecture{
        \beginsection 
        \probctr=0
        \par\noindent{\bf Lecture \number\secnumber}
        \medskip
}
\def\endlecture{\endsection\vfill\eject}
%
%
%
\def\beginlecturetitle#1{
        \beginsection 
        \probctr=0
        \par\noindent{\bf Lecture \number\secnumber : #1}
        \medskip
}
\def\endlecturetitle{\endsection\vfill\eject}
%
%
%
\def\readsec#1{\medskip{\sl Reading:} Section #1}
\def\readsecs#1{\medskip{\sl Reading:} Sections #1}
\def\hmk#1#2{\medskip{\sl Problems (due #1): }#2}
%
%       sec macro
%
\def\beginsec#1{
	\bigskip
        \beginsection 
        \par\noindent\centerline{\bf \number\secnumber . #1}
        \medskip
}
\def\endsec{\endsection\par}

\def\beginproblem{
        \advance\probctr by1
        \medbreak\par\noindent
        {\it Problem \number\secnumber .\number\probctr:\/}
}
\def\endproblem{\par\medbreak}

\def\ans{{\medskip\bold Answer: }}

\def\beginsolution{
        \medbreak\par\noindent
        {\it Solution \number\secnumber .\number\probctr:\/}
}
\def\endsolution{\par\medbreak}

\def\beginproblemset{\bigskip\hrule\bigskip\advance\leftskip by 30pt
\advance\rightskip by 30pt\smallfont}
\def\endproblemset{\bigskip\hrule\bigskip\advance\leftskip by -30pt
\advance\rightskip by -30pt\normalfont}
\def\bsp{\beginproblemset\beginproblem}
\def\esp{\endproblem\endproblemset}


%
%	some research note macros
%

\def\beginnote#1{
	%\magnification 1100
	\hsize = 5.9 true in
	\hoffset = 0.45 true in
	\baselineskip = 18pt
        \beginsection 
        \probctr=0
        \par\noindent\centerline{\bf #1}
	\centerline{filename: {\tt\jobname .tex}}
	\centerline{\today}
        \medskip
}
\def\endnote{\endsection\vskip 20pt}

%
%       These go at the beginning  of input
%
\global\newtoks\eqrtoks
\global\newtoks\thmtoks
\global\newcount\secnumber
\global\newcount\nonamectr
\global\newcount\probctr



\def\rixend{\closeout\eqroutfile \closeout\thmoutfile \vfill\eject\end}

\message{*** reference macros need to run twice to get references right ***}

